Classifying topoi in synthetic guarded domain theory

Several different topoi have played an important role in the development and applications of synthetic guarded domain theory (SGDT), a new kind of synthetic domain theory that abstracts the concept of guarded recursion frequently employed in the semantics of programming languages. In order to unify the accounts of guarded recursion and coinduction, several authors have enriched SGDT with multiple "clocks" parameterizing different time-streams, leading to more complex and difficult to understand topos models. Until now these topoi have been understood very concretely qua categories of presheaves, and the logico-geometrical question of what theories these topoi classify has remained open. We show that several important topos models of SGDT classify very simple geometric theories, and that the passage to various forms of multi-clock guarded recursion can be rephrased more compositionally in terms of the lower bagtopos construction of Vickers and variations thereon due to Johnstone. We contribute to the consolidation of SGDT by isolating the universal property of multi-clock guarded recursion as a modular construction that applies to any topos model of single-clock guarded recursion.

==> tikzlibrarycalligraphy.code.tex <==
%%
%% This is file `tikzlibrarycalligraphy.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% spath3-code.dtx  (with options: `calligraphy')
%% ----------------------------------------------------------------
%% spath3 --- Functions for manipulating PGF soft paths
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\RequirePackage{spath3}
\ExplSyntaxOn

\tl_new:N \l__cal_tmpa_tl
\tl_new:N \l__cal_tmpb_tl
\tl_new:N \l__cal_tmp_path_tl
\tl_new:N \l__cal_tmp_rpath_tl
\tl_new:N \l__cal_tmp_rpathb_tl
\tl_new:N \l__cal_tmp_patha_tl

\seq_new:N \l__cal_tmpa_seq

\int_new:N \l__cal_tmpa_int
\int_new:N \l__cal_tmpb_int
\int_new:N \g__cal_path_component_int
\int_new:N \g__cal_label_int

\fp_new:N \l__cal_tmpa_fp
\fp_new:N \l__cal_tmpb_fp
\fp_new:N \l__cal_tmpc_fp
\fp_new:N \l__cal_tmpd_fp
\fp_new:N \l__cal_tmpe_fp

\dim_new:N \l__cal_tmpa_dim
\dim_new:N \l__cal_tmpb_dim
\dim_new:N \l__cal_tmpc_dim
\dim_new:N \l__cal_tmpd_dim
\dim_new:N \l__cal_tmpe_dim
\dim_new:N \l__cal_tmpf_dim
\dim_new:N \l__cal_tmpg_dim
\dim_new:N \l__cal_tmph_dim

\bool_new:N \l__cal_annotate_bool
\bool_new:N \l__cal_taper_start_bool
\bool_new:N \l__cal_taper_end_bool
\bool_new:N \l__cal_taperable_bool

\dim_new:N \l__cal_taper_width_dim
\dim_new:N \l__cal_line_width_dim

\bool_set_true:N \l__cal_taper_start_bool
\bool_set_true:N \l__cal_taper_end_bool

\cs_generate_variant:Nn \tl_put_right:Nn {Nv}

\msg_new:nnn { calligraphy } { undefined pen } { The~ pen~ "#1"~ is~ not~ defined. }
\tikzset{
  define~pen/.code={
    \tikzset{pen~name=#1}
    \pgf@relevantforpicturesizefalse
    \tikz@addmode{
      \pgfsyssoftpath@getcurrentpath\l__cal_tmpa_tl
      \spath_components_to_seq:NV \l__cal_tmpa_seq \l__cal_tmpa_tl
      \seq_gclear_new:c {g__cal_pen_\pgfkeysvalueof{/tikz/pen~name}_seq}
      \seq_gset_eq:cN
      {g__cal_pen_\pgfkeysvalueof{/tikz/pen~name}_seq} \l__cal_tmpa_seq
      \pgfusepath{discard}%
    }
  },
  define~pen/.default={default},
  use~pen/.code={
    \tikzset{pen~name=#1}
    \int_gzero:N \g__cal_path_component_int
    \cs_set_eq:NN \pgfpathmoveto \cal_moveto:n
    \tikz@addmode{
      \pgfsyssoftpath@getcurrentpath\l__cal_tmpa_tl
      \spath_components_to_seq:NV \l__cal_tmpa_seq \l__cal_tmpa_tl
      \tl_if_exist:cTF {g__cal_pen_\pgfkeysvalueof{/tikz/pen~name}_seq}
      {
        \cal_path_create:Nc \l__cal_tmpa_seq
        {g__cal_pen_\pgfkeysvalueof{/tikz/pen~name}_seq}
      }
      {
        \msg_warning:nnx { calligraphy } { undefined pen }
        { \pgfkeysvalueof{/tikz/pen~name} }
      }
    }
  },
  use~pen/.default={default},
  pen~name/.initial={default},
  copperplate/.style={pen~name=copperplate},
  pen~colour/.initial={black},
  weight/.is~choice,
  weight/heavy/.style={
    line~width=\pgfkeysvalueof{/tikz/heavy~line~width},
    taper~width=\pgfkeysvalueof{/tikz/light~line~width},
  },
  weight/light/.style={
    line~width=\pgfkeysvalueof{/tikz/light~line~width},
    taper~width=0pt,
  },
  heavy/.style={
    weight=heavy
  },
  light/.style={
    weight=light
  },
  heavy~line~width/.initial=2pt,
  light~line~width/.initial=1pt,
  taper/.is~choice,
  taper/.default=both,
  taper/none/.style={
    taper~start=false,
    taper~end=false,
  },
  taper/both/.style={
    taper~start=true,
    taper~end=true,
  },
  taper/start/.style={
    taper~start=true,
    taper~end=false,
  },
  taper/end/.style={
    taper~start=false,
    taper~end=true,
  },
  taper~start/.code={
    \tl_if_eq:nnTF {#1} {true}
    {
      \bool_set_true:N \l__cal_taper_start_bool
    }
    {
      \bool_set_false:N \l__cal_taper_start_bool
    }
  },
  taper~start/.default={true},
  taper~end/.code={
    \tl_if_eq:nnTF {#1} {true}
    {
      \bool_set_true:N \l__cal_taper_end_bool
    }
    {
      \bool_set_false:N \l__cal_taper_end_bool
    }
  },
  taper~end/.default={true},
  taper~width/.code={\dim_set:Nn \l__cal_taper_width_dim {#1}},
  nib~style/.code~2~args={
    \tl_clear_new:c {l__cal_nib_style_#1}
    \tl_set:cn {l__cal_nib_style_#1} {#2}
  },
  stroke~style/.code~2~args={
    \tl_clear_new:c {l__cal_stroke_style_#1}
    \tl_set:cn {l__cal_stroke_style_#1} {#2}
  },
  this~stroke~style/.code={
    \tl_clear_new:c
    {l__cal_stroke_inline_style_ \int_use:N \g__cal_path_component_int}
    \tl_set:cn
    {l__cal_stroke_inline_style_ \int_use:N \g__cal_path_component_int} {#1}
  },
  annotate/.style={
    annotate~if,
    annotate~reset,
    annotation~style/.update~value={#1},
  },
  annotate~if/.default={true},
  annotate~if/.code={
    \tl_if_eq:nnTF {#1} {true}
    {
      \bool_set_true:N \l__cal_annotate_bool
    }
    {
      \bool_set_false:N \l__cal_annotate_bool
    }
  },
  annotate~reset/.code={
    \int_gzero:N \g__cal_label_int
  },
  annotation~style/.initial={draw,->},
  annotation~shift/.initial={(0,1ex)},
  every~annotation~node/.initial={anchor=south~west},
  annotation~node~style/.code~2~args={
    \tl_clear_new:c {l__cal_annotation_style_ #1 _tl}
    \tl_set:cn {l__cal_annotation_style_ #1 _tl}{#2}
  },
  tl~use:N/.code={
    \exp_args:NV \pgfkeysalso #1
  },
  tl~use:c/.code={
    \tl_if_exist:cT {#1}
    {
      \exp_args:Nv \pgfkeysalso {#1}
    }
  },
  /handlers/.update~style/.code={
    \tl_if_eq:nnF {#1} {\pgfkeysnovalue}
    {
      \pgfkeys{\pgfkeyscurrentpath/.code=\pgfkeysalso{#1}}
    }
  },
  /handlers/.update~value/.code={
    \tl_if_eq:nnF {#1} {\pgfkeysnovalue}
    {
      \pgfkeyssetvalue{\pgfkeyscurrentpath}{#1}
    }
  },
}
\NewDocumentCommand \pen { O{} }
{
  \path[define~ pen,every~ calligraphy~ pen/.try,#1]
}

\NewDocumentCommand \definepen { O{} }
{
  \tikz \path[define~ pen,every~ calligraphy~ pen/.try,#1]
}

\NewDocumentCommand \calligraphy { O{} }
{
  \path[use~ pen,every~ calligraphy/.try,#1]
}
\cs_new_protected_nopar:Npn \cal_path_create:NN #1#2
{
  \int_zero:N \l__cal_tmpa_int
  \seq_map_inline:Nn #1
  {
    \int_compare:nT {\tl_count:n {##1} > 3}
    {

      \int_incr:N \l__cal_tmpa_int
      \int_zero:N \l__cal_tmpb_int

      \tl_set:Nn \l__cal_tmp_path_tl {##1}
      \spath_open:N \l__cal_tmp_path_tl
      \spath_reverse:NV \l__cal_tmp_rpath_tl \l__cal_tmp_path_tl

      \seq_map_inline:Nn #2
      {
        \int_incr:N \l__cal_tmpb_int
        \group_begin:
        \pgfsys@beginscope
        \cal_apply_style:c {l__cal_stroke_style_ \int_use:N \l__cal_tmpa_int}
        \cal_apply_style:c {l__cal_stroke_inline_style_ \int_use:N \l__cal_tmpa_int}
        \cal_apply_style:c {l__cal_nib_style_ \int_use:N \l__cal_tmpb_int}

        \spath_initialpoint:Nn \l__cal_tmpa_tl {####1}
        \tl_set_eq:NN \l__cal_tmp_patha_tl \l__cal_tmp_path_tl
        \spath_translate:NV \l__cal_tmp_patha_tl \l__cal_tmpa_tl

        \int_compare:nTF {\tl_count:n {####1} == 3}
        {
          \cal_at_least_three:N \l__cal_tmp_patha_tl
          \spath_protocol_path:V \l__cal_tmp_patha_tl

          \tikz@options
          \dim_set:Nn \l__cal_line_width_dim {\pgflinewidth}
          \cal_maybe_taper:N \l__cal_tmp_patha_tl
        }
        {
          \spath_weld:Nn \l__cal_tmp_patha_tl {####1}
          \spath_weld:NV \l__cal_tmp_patha_tl \l__cal_tmp_rpath_tl
          \spath_reverse:Nn \l__cal_tmp_rpathb_tl {####1}
          \spath_weld:NV \l__cal_tmp_patha_tl \l__cal_tmp_rpathb_tl

          \tl_clear:N \l__cal_tmpa_tl
          \tl_set:Nn \l__cal_tmpa_tl
          {
            fill=\pgfkeysvalueof{/tikz/pen~colour},
            draw=none
          }
          \tl_if_exist:cT  {l__cal_stroke_style_ \int_use:N \l__cal_tmpa_int}
          {
            \tl_put_right:Nv \l__cal_tmpa_tl
            {l__cal_stroke_style_ \int_use:N \l__cal_tmpa_int}
          }
          \tl_if_exist:cT  {l__cal_stroke_inline_style_ \int_use:N \l__cal_tmpa_int}
          {
            \tl_put_right:Nn \l__cal_tmpa_tl {,}
            \tl_put_right:Nv \l__cal_tmpa_tl
            {l__cal_stroke_inline_style_ \int_use:N \l__cal_tmpa_int}
          }
          \tl_if_exist:cT  {l__cal_nib_style_ \int_use:N \l__cal_tmpb_int}
          {
            \tl_put_right:Nn \l__cal_tmpa_tl {,}
            \tl_put_right:Nv \l__cal_tmpa_tl
            {l__cal_nib_style_ \int_use:N \l__cal_tmpb_int}
          }
          \spath_tikz_path:VV \l__cal_tmpa_tl \l__cal_tmp_patha_tl
        }
        \pgfsys@endscope
        \group_end:
      }

      \bool_if:NT \l__cal_annotate_bool
      {
        \seq_get_right:NN #2 \l__cal_tmpa_tl
        \spath_finalpoint:NV \l__cal_tmpa_tl \l__cal_tmpa_tl
        \spath_translate:NV \l__cal_tmp_path_tl \l__cal_tmpa_tl
        \tikz@scan@one@point
        \pgfutil@firstofone
        \pgfkeysvalueof{/tikz/annotation~shift}

        \spath_translate:Nnn \l__cal_tmp_path_tl {\pgf@x} {\pgf@y}

        \pgfkeysgetvalue{/tikz/annotation~style}{\l__cal_tmpa_tl}
        \spath_tikz_path:VV \l__cal_tmpa_tl \l__cal_tmp_path_tl

        \spath_finalpoint:NV \l__cal_tmpa_tl \l__cal_tmp_path_tl

        \exp_last_unbraced:NV \pgfqpoint \l__cal_tmpa_tl
        \begin{scope}[reset~ cm]
        \node[
          every~annotation~node/.try,
          tl~use:c = {l__cal_annotation_style_ \int_use:N \l__cal_tmpa_int _tl}
        ] at (\pgf@x,\pgf@y) {\int_use:N \l__cal_tmpa_int};
        \end{scope}
      }
    }
  }
}
\cs_generate_variant:Nn \cal_path_create:NN {Nc}
\cs_new_eq:NN \cal_orig_moveto:n \pgfpathmoveto
\cs_new_nopar:Npn \cal_moveto:n #1
{
  \int_gincr:N \g__cal_path_component_int
  \cal_orig_moveto:n {#1}
}
\cs_new_nopar:Npn \cal_apply_style:N #1
{
  \tl_if_exist:NT #1 {
    \exp_args:NV \tikzset #1
  }
}
\cs_generate_variant:Nn \cal_apply_style:N {c}
\cs_new_protected_nopar:Npn \cal_at_least_three:Nn #1#2
{
  \spath_reallength:Nn \l__cal_tmpa_int {#2}
  \tl_clear:N \l__cal_tmpb_tl
  \tl_set:Nn \l__cal_tmpb_tl {#2}
  \int_compare:nTF {\l__cal_tmpa_int = 1}
  {
    \spath_split_at:Nn \l__cal_tmpb_tl {2/3}
    \spath_split_at:Nn \l__cal_tmpb_tl {1/2}
  }
  {
    \int_compare:nT {\l__cal_tmpa_int = 2}
    {
      \spath_split_at:Nn \l__cal_tmpb_tl {1.5}
      \spath_split_at:Nn \l__cal_tmpb_tl {.5}
    }
  }
  \tl_set_eq:NN #1 \l__cal_tmpb_tl
}
\cs_generate_variant:Nn \cal_at_least_three:Nn {NV}
\cs_new_protected_nopar:Npn \cal_at_least_three:N #1
{
  \cal_at_least_three:NV #1#1
}
\cs_generate_variant:Nn \cal_at_least_three:N {c}
\cs_new_protected_nopar:Npn \cal_maybe_taper:N #1
{
  \tl_set_eq:NN \l__cal_tmpa_tl #1

  \bool_if:NT \l__cal_taper_start_bool
  {

    \dim_set:Nn \l__cal_tmpa_dim {\tl_item:Nn \l__cal_tmpa_tl {2}}
    \dim_set:Nn \l__cal_tmpb_dim {\tl_item:Nn \l__cal_tmpa_tl {3}}
    \tl_set:Nx \l__cal_tmpb_tl {\tl_item:Nn \l__cal_tmpa_tl {4}}

    \tl_case:NnF \l__cal_tmpb_tl
    {
      \c_spath_lineto_tl
      {

        \bool_set_true:N \l__cal_taperable_bool
        \dim_set:Nn \l__cal_tmpg_dim {\tl_item:Nn \l__cal_tmpa_tl {5}}
        \dim_set:Nn \l__cal_tmph_dim {\tl_item:Nn \l__cal_tmpa_tl {6}}
        \dim_set:Nn \l__cal_tmpc_dim {(2\l__cal_tmpa_dim + \l__cal_tmpg_dim)/3}
        \dim_set:Nn \l__cal_tmpd_dim {(2\l__cal_tmpb_dim + \l__cal_tmph_dim)/3}
        \dim_set:Nn \l__cal_tmpe_dim {(\l__cal_tmpa_dim + 2\l__cal_tmpg_dim)/3}
        \dim_set:Nn \l__cal_tmpf_dim {(\l__cal_tmpb_dim + 2\l__cal_tmph_dim)/3}
        \prg_replicate:nn {4}
        {
          \tl_set:Nx \l__cal_tmpa_tl {\tl_tail:N \l__cal_tmpa_tl}
        }
        \tl_put_left:NV \l__cal_tmpa_tl \c_spath_moveto_tl
      }
      \c_spath_curvetoa_tl
      {
        \bool_set_true:N \l__cal_taperable_bool
        \dim_set:Nn \l__cal_tmpc_dim {\tl_item:Nn \l__cal_tmpa_tl {5}}
        \dim_set:Nn \l__cal_tmpd_dim {\tl_item:Nn \l__cal_tmpa_tl {6}}
        \dim_set:Nn \l__cal_tmpe_dim {\tl_item:Nn \l__cal_tmpa_tl {8}}
        \dim_set:Nn \l__cal_tmpf_dim {\tl_item:Nn \l__cal_tmpa_tl {9}}
        \dim_set:Nn \l__cal_tmpg_dim {\tl_item:Nn \l__cal_tmpa_tl {11}}
        \dim_set:Nn \l__cal_tmph_dim {\tl_item:Nn \l__cal_tmpa_tl {12}}
        \prg_replicate:nn {10}
        {
          \tl_set:Nx \l__cal_tmpa_tl {\tl_tail:N \l__cal_tmpa_tl}
        }
        \tl_put_left:NV \l__cal_tmpa_tl \c_spath_moveto_tl
      }
    }
    {
      \bool_set_false:N \l__cal_taperable_bool
    }

    \bool_if:NT \l__cal_taperable_bool
    {
      \__cal_taper_aux:
    }

  }

  \bool_if:NT \l__cal_taper_end_bool
  {

    \dim_set:Nn \l__cal_tmpa_dim {\tl_item:Nn \l__cal_tmpa_tl {-2}}
    \dim_set:Nn \l__cal_tmpb_dim {\tl_item:Nn \l__cal_tmpa_tl {-1}}
    \tl_set:Nx \l__cal_tmpb_tl {\tl_item:Nn \l__cal_tmpa_tl {-3}}

    \tl_case:NnF \l__cal_tmpb_tl
    {
      \c_spath_lineto_tl
      {

        \bool_set_true:N \l__cal_taperable_bool
        \dim_set:Nn \l__cal_tmpg_dim {\tl_item:Nn \l__cal_tmpa_tl {-5}}
        \dim_set:Nn \l__cal_tmph_dim {\tl_item:Nn \l__cal_tmpa_tl {-4}}
        \dim_set:Nn \l__cal_tmpc_dim {(2\l__cal_tmpa_dim + \l__cal_tmpg_dim)/3}
        \dim_set:Nn \l__cal_tmpd_dim {(2\l__cal_tmpb_dim + \l__cal_tmph_dim)/3}
        \dim_set:Nn \l__cal_tmpe_dim {(\l__cal_tmpa_dim + 2\l__cal_tmpg_dim)/3}
        \dim_set:Nn \l__cal_tmpf_dim {(\l__cal_tmpb_dim + 2\l__cal_tmph_dim)/3}
        \tl_reverse:N \l__cal_tmpa_tl
        \prg_replicate:nn {3}
        {
          \tl_set:Nx \l__cal_tmpa_tl {\tl_tail:N \l__cal_tmpa_tl}
        }
        \tl_reverse:N \l__cal_tmpa_tl
      }
      \c_spath_curveto_tl
      {
        \bool_set_true:N \l__cal_taperable_bool
        \dim_set:Nn \l__cal_tmpc_dim {\tl_item:Nn \l__cal_tmpa_tl {-5}}
        \dim_set:Nn \l__cal_tmpd_dim {\tl_item:Nn \l__cal_tmpa_tl {-4}}
        \dim_set:Nn \l__cal_tmpe_dim {\tl_item:Nn \l__cal_tmpa_tl {-8}}
        \dim_set:Nn \l__cal_tmpf_dim {\tl_item:Nn \l__cal_tmpa_tl {-7}}
        \dim_set:Nn \l__cal_tmpg_dim {\tl_item:Nn \l__cal_tmpa_tl {-11}}
        \dim_set:Nn \l__cal_tmph_dim {\tl_item:Nn \l__cal_tmpa_tl {-10}}
        \tl_reverse:N \l__cal_tmpa_tl
        \prg_replicate:nn {9}
        {
          \tl_set:Nx \l__cal_tmpa_tl {\tl_tail:N \l__cal_tmpa_tl}
        }
        \tl_reverse:N \l__cal_tmpa_tl
      }
    }
    {
      \bool_set_false:N \l__cal_taperable_bool
    }

    \bool_if:NT \l__cal_taperable_bool
    {
      \__cal_taper_aux:
    }

  }

  \pgfsyssoftpath@setcurrentpath\l__cal_tmpa_tl
  \pgfsetstrokecolor{\pgfkeysvalueof{/tikz/pen~colour}}
  \pgfusepath{stroke}

}
\cs_new_protected_nopar:Npn \__cal_taper_aux:
{
  \tl_clear:N \l__cal_tmpb_tl
  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_moveto_tl

  \fp_set:Nn \l__cal_tmpa_fp
  {
    \l__cal_tmpd_dim - \l__cal_tmpb_dim
  }
  \fp_set:Nn \l__cal_tmpb_fp
  {
    \l__cal_tmpa_dim - \l__cal_tmpc_dim
  }
  \fp_set:Nn \l__cal_tmpe_fp
  {
    (\l__cal_tmpa_fp^2 + \l__cal_tmpb_fp^2)^.5
  }

  \fp_set:Nn \l__cal_tmpa_fp
  {
    .5*\l__cal_taper_width_dim
    *
    \l__cal_tmpa_fp / \l__cal_tmpe_fp
  }
  \fp_set:Nn \l__cal_tmpb_fp
  {
    .5*\l__cal_taper_width_dim
    *
    \l__cal_tmpb_fp / \l__cal_tmpe_fp
  }

  \fp_set:Nn \l__cal_tmpc_fp
  {
    \l__cal_tmph_dim - \l__cal_tmpf_dim
  }
  \fp_set:Nn \l__cal_tmpd_fp
  {
    \l__cal_tmpe_dim - \l__cal_tmpg_dim
  }
  \fp_set:Nn \l__cal_tmpe_fp
  {
    (\l__cal_tmpc_fp^2 + \l__cal_tmpd_fp^2)^.5
  }

  \fp_set:Nn \l__cal_tmpc_fp
  {
    .5*\l__cal_line_width_dim
    *
    \l__cal_tmpc_fp / \l__cal_tmpe_fp
  }
  \fp_set:Nn \l__cal_tmpd_fp
  {
    .5*\l__cal_line_width_dim
    *
    \l__cal_tmpd_fp / \l__cal_tmpe_fp
  }

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpa_dim}}
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpb_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetoa_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpc_dim}}
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpd_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetob_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpc_fp + \l__cal_tmpe_dim}}
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpd_fp + \l__cal_tmpf_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curveto_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpc_fp + \l__cal_tmpg_dim}}
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpd_fp + \l__cal_tmph_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetoa_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {
      \dim_eval:n
      {
        \fp_to_dim:N \l__cal_tmpc_fp + \l__cal_tmpg_dim
        - \fp_to_dim:n{ 1.32 * \l__cal_tmpd_fp
        }
      }
    }
    {
      \dim_eval:n
      {
        \fp_to_dim:N \l__cal_tmpd_fp + \l__cal_tmph_dim
        + \fp_to_dim:n {1.32* \l__cal_tmpc_fp
        }
      }
    }
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetob_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {
      \dim_eval:n
      {
        -\fp_to_dim:N \l__cal_tmpc_fp + \l__cal_tmpg_dim
        - \fp_to_dim:n {1.32 * \l__cal_tmpd_fp
        }
      }
    }
    {
      \dim_eval:n
      {
        -\fp_to_dim:N \l__cal_tmpd_fp + \l__cal_tmph_dim
        + \fp_to_dim:n {1.32 * \l__cal_tmpc_fp
        }
      }
    }
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curveto_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpc_fp + \l__cal_tmpg_dim}}
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpd_fp + \l__cal_tmph_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetoa_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpc_fp + \l__cal_tmpe_dim}}
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpd_fp + \l__cal_tmpf_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetob_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpc_dim}}
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpd_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curveto_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpa_dim}}
    {\dim_eval:n { -\fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpb_dim}}
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetoa_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {
      \dim_eval:n
      {
        -\fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpa_dim
        + \fp_to_dim:n{ 1.32 * \l__cal_tmpb_fp}
      }
    }
    {
      \dim_eval:n
      {
        -\fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpb_dim
        - \fp_to_dim:n {1.32* \l__cal_tmpa_fp}
      }
    }
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curvetob_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {
      \dim_eval:n
      {
        \fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpa_dim
        + \fp_to_dim:n {1.32 * \l__cal_tmpb_fp}
      }
    }
    {
      \dim_eval:n
      {
        \fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpb_dim
        - \fp_to_dim:n {1.32 * \l__cal_tmpa_fp}
      }
    }
  }

  \tl_put_right:NV \l__cal_tmpb_tl \c_spath_curveto_tl

  \tl_put_right:Nx \l__cal_tmpb_tl
  {
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpa_fp + \l__cal_tmpa_dim}}
    {\dim_eval:n { \fp_to_dim:N \l__cal_tmpb_fp + \l__cal_tmpb_dim}}
  }

  \pgfsyssoftpath@setcurrentpath\l__cal_tmpb_tl
  \pgfsetfillcolor{\pgfkeysvalueof{/tikz/pen~colour}}
  \pgfusepath{fill}
}
\tl_set:Nn \l__cal_tmpa_tl {\pgfsyssoftpath@movetotoken{0pt}{0pt}}
\spath_components_to_seq:NV \l__cal_tmpa_seq \l__cal_tmpa_tl
\seq_gclear_new:N \g__cal_pen_copperplate_seq
\seq_gset_eq:NN \g__cal_pen_copperplate_seq \l__cal_tmpa_seq
\DeclareDocumentCommand \CopperplatePath { m }
{
  \spath_components_to_seq:NV \l__cal_tmpa_seq #1
  \cal_path_create:NN \l__cal_tmpa_seq \g__cal_pen_copperplate_seq
}
\ExplSyntaxOff
\expandafter\ifx\csname pgfdeclaredecoration\endcsname\relax
\else
\pgfdeclaredecoration{calligraphic brace}{brace}%
{%
  \state{brace}[width=+\pgfdecoratedremainingdistance,next state=final]%
  {%
    \pgfsyssoftpath@setcurrentpath{\pgfutil@empty}%
    \pgfpathmoveto{\pgfpointorigin}%
    \pgfpathcurveto%
    {%
      \pgfqpoint%
      {.15\pgfdecorationsegmentamplitude}%
      {.3\pgfdecorationsegmentamplitude}%
    }%
    {%
      \pgfqpoint%
      {.5\pgfdecorationsegmentamplitude}%
      {.5\pgfdecorationsegmentamplitude}%
    }%
    {%
      \pgfqpoint%
      {\pgfdecorationsegmentamplitude}%
      {.5\pgfdecorationsegmentamplitude}%
    }%
    {%
      \pgftransformxshift%
      {+\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance}%
      \pgfpathlineto%
      {%
        \pgfqpoint%
        {-\pgfdecorationsegmentamplitude}%
        {.5\pgfdecorationsegmentamplitude}%
      }%
      \pgfpathcurveto
      {%
        \pgfqpoint%
        {-.5\pgfdecorationsegmentamplitude}%
        {.5\pgfdecorationsegmentamplitude}%
      }%
      {%
        \pgfqpoint%
        {-.15\pgfdecorationsegmentamplitude}%
        {.7\pgfdecorationsegmentamplitude}%
      }%
      {%
        \pgfqpoint%
        {0\pgfdecorationsegmentamplitude}%
        {1\pgfdecorationsegmentamplitude}%
      }%
      \pgfpathmoveto%
      {%
        \pgfqpoint%
        {0\pgfdecorationsegmentamplitude}%
        {1\pgfdecorationsegmentamplitude}%
      }%
      \pgfpathcurveto%
      {%
        \pgfqpoint%
        {.15\pgfdecorationsegmentamplitude}%
        {.7\pgfdecorationsegmentamplitude}%
      }%
      {%
        \pgfqpoint%
        {.5\pgfdecorationsegmentamplitude}%
        {.5\pgfdecorationsegmentamplitude}%
      }%
      {%
        \pgfqpoint%
        {\pgfdecorationsegmentamplitude}%
        {.5\pgfdecorationsegmentamplitude}%
      }%
    }%
    {%
      \pgftransformxshift{+\pgfdecoratedremainingdistance}%
      \pgfpathlineto%
      {%
        \pgfqpoint%
        {-\pgfdecorationsegmentamplitude}%
        {.5\pgfdecorationsegmentamplitude}%
      }%
      \pgfpathcurveto%
      {%
        \pgfqpoint%
        {-.5\pgfdecorationsegmentamplitude}%
        {.5\pgfdecorationsegmentamplitude}%
      }%
      {%
        \pgfqpoint%
        {-.15\pgfdecorationsegmentamplitude}%
        {.3\pgfdecorationsegmentamplitude}%
      }%
      {\pgfqpoint{0pt}{0pt}}%
    }%
    \tikzset{%
      taper width=.5\pgflinewidth,%
      taper%
    }%%
    \pgfsyssoftpath@getcurrentpath\cal@tmp@path%
    \CopperplatePath{\cal@tmp@path}%
  }%
  \state{final}{}%
}%
\pgfdeclaredecoration{calligraphic straight parenthesis}{brace}
{
  \state{brace}[width=+\pgfdecoratedremainingdistance,next state=final]%
  {%
    \pgfsyssoftpath@setcurrentpath{\pgfutil@empty}%
    \pgfpathmoveto{\pgfpointorigin}%
    \pgfpathcurveto%
    {%
      \pgfqpoint%
      {.76604\pgfdecorationsegmentamplitude}%
      {.64279\pgfdecorationsegmentamplitude}%
    }%
    {%
      \pgfqpoint%
      {2.3333\pgfdecorationsegmentamplitude}%
      {\pgfdecorationsegmentamplitude}%
    }%
    {%
      \pgfqpoint%
      {3.3333\pgfdecorationsegmentamplitude}%
      {\pgfdecorationsegmentamplitude}%
    }%
    {%
      \pgftransformxshift{+\pgfdecoratedremainingdistance}%
      \pgfpathlineto%
      {%
        \pgfqpoint%
        {-3.3333\pgfdecorationsegmentamplitude}%
        {\pgfdecorationsegmentamplitude}%
      }%
      \pgfpathcurveto%
      {%
        \pgfqpoint%
        {-2.3333\pgfdecorationsegmentamplitude}%
        {\pgfdecorationsegmentamplitude}%
      }%
      {%
        \pgfqpoint%
        {-.76604\pgfdecorationsegmentamplitude}%
        {.64279\pgfdecorationsegmentamplitude}%
      }%
      {\pgfqpoint{0pt}{0pt}}%
    }%
    \tikzset{%
      taper width=.5\pgflinewidth,%
      taper%
    }%
    \pgfsyssoftpath@getcurrentpath\cal@tmp@path%
    \CopperplatePath{\cal@tmp@path}%
  }%
  \state{final}{}%
}
\pgfdeclaredecoration{calligraphic curved parenthesis}{brace}
{
  \state{brace}[width=+\pgfdecoratedremainingdistance,next state=final]%
  {%
    \pgfsyssoftpath@setcurrentpath{\pgfutil@empty}%
    \pgfpathmoveto{\pgfpointorigin}%
    \pgf@xa=\pgfdecoratedremainingdistance\relax%
    \advance\pgf@xa by -1.5890\pgfdecorationsegmentamplitude\relax%
    \edef\cgrphy@xa{\the\pgf@xa}%
    \pgfpathcurveto%
    {%
      \pgfqpoint%
      {1.5890\pgfdecorationsegmentamplitude}%
      {1.3333\pgfdecorationsegmentamplitude}%
    }%
    {\pgfqpoint{\cgrphy@xa}{1.3333\pgfdecorationsegmentamplitude}}%
    {\pgfqpoint{\pgfdecoratedremainingdistance}{0pt}}%
    \tikzset{%
      taper width=.5\pgflinewidth,%
      taper%
    }%
    \pgfsyssoftpath@getcurrentpath\cal@tmp@path%
    \CopperplatePath{\cal@tmp@path}%
  }%
  \state{final}{}%
}
\fi
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  spath3_code.dtx
%%                                  calligraphy_doc.tex
%%                                  knots_doc.tex
%%                                  spath3.tex
%% and the derived files            spath3.ins,
%%                                  spath3_code.pdf,
%%                                  spath3.sty,
%%                                  tikzlibrarycalligraphy.code.tex
%%                                  tikzlibraryknots.code.tex
%%                                  tikzlibraryspath3.code.tex
%%                                  calligraphy.pdf
%%                                  knots.pdf
%%                                  spath3.pdf
%%                                  README
%% 
%%
%% End of file `tikzlibrarycalligraphy.code.tex'.


==> tikzlibraryknots.code.tex <==
%%
%% This is file `tikzlibraryknots.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% spath3-code.dtx  (with options: `knots')
%% ----------------------------------------------------------------
%% spath3 --- Functions for manipulating PGF soft paths
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
%%
\RequirePackage{spath3}
\usetikzlibrary{intersections,spath3}

\ExplSyntaxOn

\tl_new:N \l__knot_tmpa_tl
\tl_new:N \l__knot_tmpb_tl
\tl_new:N \l__knot_tmpc_tl
\tl_new:N \l__knot_tmpd_tl
\tl_new:N \l__knot_tmpg_tl
\tl_new:N \l__knot_redraws_tl
\tl_new:N \l__knot_clip_width_tl
\tl_new:N \l__knot_name_tl
\tl_new:N \l__knot_node_tl
\tl_new:N \l__knot_aux_tl
\tl_new:N \l__knot_auxa_tl
\tl_new:N \l__knot_prefix_tl

\seq_new:N \l__knot_segments_seq

\int_new:N \l__knot_tmpa_int
\int_new:N \l__knot_strands_int
\int_new:N \g__knot_intersections_int
\int_new:N \g__knot_filaments_int
\int_new:N \l__knot_component_start_int

\fp_new:N \l__knot_tmpa_fp
\fp_new:N \l__knot_tmpb_fp

\dim_new:N \l__knot_tmpa_dim
\dim_new:N \l__knot_tmpb_dim
\dim_new:N \l__knot_tolerance_dim
\dim_new:N \l__knot_redraw_tolerance_dim
\dim_new:N \l__knot_clip_bg_radius_dim
\dim_new:N \l__knot_clip_draw_radius_dim

\bool_new:N \l__knot_draft_bool
\bool_new:N \l__knot_ignore_ends_bool
\bool_new:N \l__knot_self_intersections_bool
\bool_new:N \l__knot_splits_bool
\bool_new:N \l__knot_super_draft_bool

\bool_new:N \l__knot_prepend_prev_bool
\bool_new:N \l__knot_append_next_bool
\bool_new:N \l__knot_skip_bool
\bool_new:N \l__knot_save_bool
\bool_new:N \l__knot_debugging_bool

\seq_new:N \g__knot_nodes_seq

\bool_set_true:N \l__knot_ignore_ends_bool
\tikzset{
  spath/prefix/knot/.style={
    spath/set~ prefix=knot strand,
  },
  spath/suffix/knot/.style={
    spath/set~ suffix={},
  },
  knot/.code={
    \tl_if_eq:nnTF {#1} {none}
    {
      \tikz@addmode{\tikz@mode@doublefalse}
    }
    {
      \tikz@addmode{\tikz@mode@doubletrue}
      \tl_if_eq:nnTF {\pgfkeysnovalue} {#1}
      {
        \tikz@addoption{\pgfsetinnerstrokecolor{.}}
      }
      {
        \pgfsetinnerstrokecolor{#1}
      }
      \tikz@addoption{
        \pgfsetstrokecolor{knotbg}
      }
      \tl_set:Nn \tikz@double@setup{
        \pgfsetinnerlinewidth{\pgflinewidth}
        \pgfsetlinewidth{\dim_eval:n {\tl_use:N \l__knot_gap_tl \pgflinewidth}}
      }
    }
  },
  knot~ gap/.store~ in=\l__knot_gap_tl,
  knot~ gap=3,
  knot~ diagram/.is~family,
  knot~ diagram/.unknown/.code={
    \tl_set_eq:NN \l__knot_tmpa_tl \pgfkeyscurrentname
    \pgfkeysalso{
      /tikz/\l__knot_tmpa_tl=#1
    }
  },
  background~ colour/.code={%
    \colorlet{knotbg}{#1}%
  },
  background~ color/.code={%
    \colorlet{knotbg}{#1}%
  },
  background~ colour=white,
  knot~ diagram,
  name/.store~ in=\l__knot_name_tl,
  name={knot},
  save~ intersections/.is~ choice,
  save~ intersections/.default=true,
  save~ intersections/true/.code={
    \bool_set_true:N \l__knot_save_bool
  },
  save~ intersections/false/.code={
    \bool_set_false:N \l__knot_save_bool
  },
  every~ strand/.style={draw},
  ignore~ endpoint~ intersections/.code={
    \tl_if_eq:nnTF {#1} {true}
    {
      \bool_set_true:N \l__knot_ignore_ends_bool
    }
    {
      \bool_set_false:N \l__knot_ignore_ends_bool
    }
  },
  ignore~ endpoint~ intersections/.default=true,
  consider~ self~ intersections/.is~choice,
  consider~ self~ intersections/true/.code={
    \bool_set_true:N \l__knot_self_intersections_bool
    \bool_set_true:N \l__knot_splits_bool
  },
  consider~ self~ intersections/false/.code={
    \bool_set_false:N \l__knot_self_intersections_bool
    \bool_set_false:N \l__knot_splits_bool
  },
  consider~ self~ intersections/no~ splits/.code={
    \bool_set_true:N \l__knot_self_intersections_bool
    \bool_set_false:N \l__knot_splits_bool
  },
  consider~ self~ intersections/.default={true},
  clip~ radius/.code={
    \dim_set:Nn \l__knot_clip_bg_radius_dim {#1}
    \dim_set:Nn \l__knot_clip_draw_radius_dim {#1+2pt}
  },
  clip~ draw~ radius/.code={
    \dim_set:Nn \l__knot_clip_draw_radius_dim {#1}
  },
  clip~ background~ radius/.code={
    \dim_set:Nn \l__knot_clip_bg_radius_dim {#1}
  },
  clip~ radius=10pt,
  end~ tolerance/.code={
    \dim_set:Nn \l__knot_tolerance_dim {#1}
  },
  end~ tolerance=14pt,
  clip/.style={
    clip
  },
  background~ clip/.style={
    clip
  },
  clip~ width/.code={
    \tl_set:Nn \l__knot_clip_width_tl {#1}
  },
  clip~ width=3,
  flip~ crossing/.code={%
    \tl_clear_new:c {l__knot_crossing_#1}
    \tl_set:cn {l__knot_crossing_#1} {x}
  },
  ignore~ crossing/.code={%
    \tl_clear_new:c {l__knot_ignore_crossing_#1}
    \tl_set:cn {l__knot_ignore_crossing_#1} {x}
  },
  draft~ mode/.is~ choice,
  draft~ mode/off/.code={%
    \bool_set_false:N \l__knot_draft_bool
    \bool_set_false:N \l__knot_super_draft_bool
  },
  draft~ mode/crossings/.code={%
    \bool_set_true:N \l__knot_draft_bool
    \bool_set_false:N \l__knot_super_draft_bool
  },
  draft~ mode/strands/.code={%
    \bool_set_true:N \l__knot_draft_bool
    \bool_set_true:N \l__knot_super_draft_bool
  },
  debug/.is~ choice,
  debug/true/.code={
    \bool_set_true:N \l__knot_debugging_bool
  },
  debug/false/.code={
    \bool_set_false:N \l__knot_debugging_bool
  },
  debug/.default=true,
  draft/.is~ family,
  draft,
  crossing~ label/.style={
    overlay,
    fill=white,
    fill~ opacity=.5,
    text~ opacity=1,
    text=blue,
    pin~ edge={blue,<-}
  },
  strand~ label/.style={
    overlay,
    circle,
    draw=purple,
    fill=white,
    fill~ opacity=.5,
    text~ opacity=1,
    text=purple,
    inner~ sep=0pt
  },
}
\cs_new_nopar:Npn \knot_debug:n #1
{
  \bool_if:NT \l__knot_debugging_bool
  {
    \iow_term:n {===Knot~ debug: #1===}
  }
}

\cs_generate_variant:Nn \knot_debug:n {x}
\cs_new_nopar:Npn \knot_apply_style:N #1
{
  \knot_debug:n {knot~ apply~ style}
  \tl_if_exist:NT #1 {
    \exp_args:NV \tikzset #1
  }
}
\cs_generate_variant:Nn \knot_apply_style:N {c}
\NewDocumentCommand \flipcrossings {m}
{
  \tikzset{knot~ diagram/flip~ crossing/.list={#1}}%
}
\NewDocumentCommand \strand { O{} }
{
  \int_incr:N \l__knot_strands_int
  \tl_clear_new:c {l__knot_options_strand \int_use:N \l__knot_strands_int}
  \tl_set:cn {l__knot_options_strand \int_use:N \l__knot_strands_int} {#1}
  \path[#1,spath/set~ name=knot,spath/save=\int_use:N \l__knot_strands_int]
}
\NewDocumentEnvironment{knot} { O{} }
{
  \knot_initialise:n {#1}
}
{
  \knot_render:
}
\cs_new_protected_nopar:Npn \knot_initialise:n #1
{
  \knot_debug:n {knot~ initialise}
  \tikzset{knot~ diagram/.cd,every~ knot~ diagram/.try,#1}
  \int_zero:N \l__knot_strands_int
  \tl_clear:N \l__knot_redraws_tl
  \seq_gclear:N \g__knot_nodes_seq
}
\cs_new_protected_nopar:Npn \knot_render:
{
  \knot_debug:n {knot~ render}
  \pgfscope
  \pgftransformreset
  \dim_set:Nn \l__knot_redraw_tolerance_dim {\fp_to_dim:n
    {
      sqrt(2) * max(\l__knot_clip_bg_radius_dim, \l__knot_clip_draw_radius_dim)
    }
  }
  \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_draw_strand:n
  \bool_if:NF \l__knot_super_draft_bool
  {
    \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_draw_labels:n
    \bool_if:NTF \l__knot_self_intersections_bool
    {
      \knot_split_strands:
      \int_set_eq:NN \l__knot_tmpa_int \g__knot_filaments_int
      \tl_set:Nn \l__knot_prefix_tl {filament}
    }
    {
      \int_set_eq:NN \l__knot_tmpa_int \l__knot_strands_int
      \tl_set:Nn \l__knot_prefix_tl {strand}
    }
    \int_gzero:N \g__knot_intersections_int
    \tl_clear:N \l__knot_node_tl
    \bool_if:NT \l__knot_draft_bool
    {
      \tl_set:Nn \l__knot_node_tl {
        \exp_not:N \node[coordinate,
          pin={[
              node~ contents={\int_use:N \g__knot_intersections_int},
              knot~ diagram/draft/crossing~ label,
              knot~ diagram/draft/crossing~
              \int_use:N \g__knot_intersections_int \c_space_tl label/.try
            ]
            }]
      }
    }
    \int_step_variable:nnnNn {1} {1} {\l__knot_tmpa_int - 1} \l__knot_tmpa_tl
    {
      \int_step_variable:nnnNn
      {\tl_use:N \l__knot_tmpa_tl + 1}
      {1}
      {\l__knot_tmpa_int} \l__knot_tmpb_tl
      {
        \knot_intersections:VV \l__knot_tmpa_tl \l__knot_tmpb_tl
      }
    }
    \tl_use:N \l__knot_redraws_tl
    \seq_use:Nn \g__knot_nodes_seq {}
  }
  \endpgfscope
  \knot_debug:x {knot~rendered,
    ~found~\int_use:N  \g__knot_intersections_int \c_space_tl~intersections}
}
\cs_new_protected_nopar:Npn \knot_draw_strand:n #1
{
  \knot_debug:n {knot~ draw~ strand~ #1}
  \pgfscope
  \group_begin:
  \spath_bake_round:c {knot strand #1}
  \tl_set:Nn \l__knot_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_put_right:Nv \l__knot_tmpa_tl {l__knot_options_strand #1}
  \tl_put_right:Nn \l__knot_tmpa_tl
  {
    ,
    knot~ diagram/only~ when~ rendering/.try,
    only~ when~ rendering/.try,
  }
  \spath_tikz_path:Vv \l__knot_tmpa_tl {knot strand #1}
  \group_end:
  \endpgfscope
}
\cs_generate_variant:Nn \tl_put_right:Nn {Nv}
\cs_new_protected_nopar:Npn \knot_draw_labels:n #1
{
  \knot_debug:n {knot~ draw~ labels}
  \bool_if:NT \l__knot_draft_bool
  {
    \spath_finalpoint:Nv \l__knot_tmpb_tl {knot strand #1}
    \dim_set:Nn \l__knot_tmpa_dim {\tl_item:Nn \l__knot_tmpb_tl {1}}
    \dim_set:Nn \l__knot_tmpb_dim {\tl_item:Nn \l__knot_tmpb_tl {2}}
    \node[
      knot~ diagram/draft/strand~label
    ] at (\l__knot_tmpa_dim,\l__knot_tmpb_dim) {#1};
    \spath_initialpoint:Nv \l__knot_tmpb_tl {knot strand #1}
    \dim_set:Nn \l__knot_tmpa_dim {\tl_item:Nn \l__knot_tmpb_tl {1}}
    \dim_set:Nn \l__knot_tmpb_dim {\tl_item:Nn \l__knot_tmpb_tl {2}}
    \node[
      knot~ diagram/draft/strand~label
    ] at (\l__knot_tmpa_dim,\l__knot_tmpb_dim) {#1};
  }
  \bool_if:nT {
    \l__knot_self_intersections_bool
    &&
    \l__knot_splits_bool
  }
  {
    \tl_clear:N \l__knot_tmpa_tl
    \spath_initialpoint:Nv \l__knot_tmpa_tl {knot strand #1}
    \tl_put_left:NV \l__knot_tmpa_tl \c_spath_moveto_tl
    \spath_segments_to_seq:Nv \l__knot_segments_seq {knot strand #1}
    \seq_map_function:NN \l__knot_segments_seq \knot_split_self_intersects:N
    \tl_set_eq:cN {knot strand #1} \l__knot_tmpa_tl
  }
}
\cs_new_protected_nopar:Npn \knot_split_self_intersects:N #1
{
  \knot_debug:n {knot~ split~ self~ intersects}
  \tl_set:Nx \l__knot_tmpc_tl {\tl_item:nn {#1} {4}}
  \tl_case:NnF \l__knot_tmpc_tl
  {
    \c_spath_curvetoa_tl
    {
      \fp_set:Nn \l__knot_tmpa_fp
      {
        (\tl_item:nn {#1} {3} - 3 * \tl_item:nn {#1} {6}
        + 3 * \tl_item:nn {#1} {9} - \tl_item:nn {#1} {12})
        *
        (3 * \tl_item:nn {#1} {8} - 3 * \tl_item:nn {#1} {11})
        -
        (\tl_item:nn {#1} {2} - 3 * \tl_item:nn {#1} {5}
        + 3 * \tl_item:nn {#1} {8} - \tl_item:nn {#1} {11})
        *
        (3 * \tl_item:nn {#1} {9} - 3 * \tl_item:nn {#1} {12})
      }
      \fp_set:Nn \l__knot_tmpb_fp
      {
        (\tl_item:nn {#1} {2} - 3 * \tl_item:nn {#1} {5}
        + 3 * \tl_item:nn {#1} {8} - \tl_item:nn {#1} {11})
        *
        (3 * \tl_item:nn {#1} {6} - 6 * \tl_item:nn {#1} {9}
        + 3 * \tl_item:nn {#1} {12})
        -
        (\tl_item:nn {#1} {3} - 3 * \tl_item:nn {#1} {6}
        + 3 * \tl_item:nn {#1} {9} - \tl_item:nn {#1} {12})
        *
        (3 * \tl_item:nn {#1} {5} - 6 * \tl_item:nn {#1} {8}
        + 3 * \tl_item:nn {#1} {11})
      }
      \fp_compare:nTF
      {
        \l__knot_tmpb_fp != 0
      }
      {
        \fp_set:Nn \l__knot_tmpa_fp {.5 * \l__knot_tmpa_fp / \l__knot_tmpb_fp}
        \bool_if:nTF
        {
          \fp_compare_p:n {0 < \l__knot_tmpa_fp}
          &&
          \fp_compare_p:n {\l__knot_tmpa_fp < 1}
        }
        {
          \spath_split_curve:NNnV
          \l__knot_tmpc_tl
          \l__knot_tmpd_tl
          {#1}
          \l__knot_tmpa_fp
          \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
          \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
          \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
          \tl_set:Nx \l__knot_tmpd_tl {\tl_tail:N \l__knot_tmpd_tl}
          \tl_set:Nx \l__knot_tmpd_tl {\tl_tail:N \l__knot_tmpd_tl}
          \tl_set:Nx \l__knot_tmpd_tl {\tl_tail:N \l__knot_tmpd_tl}
          \tl_put_right:NV \l__knot_tmpa_tl \l__knot_tmpc_tl
          \tl_put_right:NV \l__knot_tmpa_tl \l__knot_tmpd_tl
        }
        {
          \tl_set:Nn \l__knot_tmpc_tl {#1}
          \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
          \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
          \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
          \tl_put_right:NV \l__knot_tmpa_tl \l__knot_tmpc_tl
        }
      }
      {
        \tl_set:Nn \l__knot_tmpc_tl {#1}
        \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
        \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
        \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
        \tl_put_right:NV \l__knot_tmpa_tl \l__knot_tmpc_tl
      }
    }
    \c_spath_lineto_tl
    {
      \tl_set:Nn \l__knot_tmpc_tl {#1}
      \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
      \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
      \tl_set:Nx \l__knot_tmpc_tl {\tl_tail:N \l__knot_tmpc_tl}
      \tl_put_right:NV \l__knot_tmpa_tl \l__knot_tmpc_tl
    }
  }
  {
    \tl_put_right:Nn \l__knot_tmpa_tl {#1}
  }
}
\cs_new_protected_nopar:Npn \knot_intersections:nn #1#2
{
  \knot_debug:x {knot~ intersections~ between~
    \l__knot_prefix_tl \c_space_tl #1~ and~ #2}
  \group_begin:
  \tl_set_eq:NN \l__knot_tmpa_tl \l__knot_prefix_tl
  \tl_put_right:Nn \l__knot_tmpa_tl {#1}
  \tl_set_eq:NN \l__knot_tmpb_tl \l__knot_prefix_tl
  \tl_put_right:Nn \l__knot_tmpb_tl {#2}
  \tl_set_eq:Nc \l__knot_tmpc_tl {knot \tl_use:N \l__knot_tmpa_tl}
  \tl_set_eq:Nc \l__knot_tmpd_tl {knot \tl_use:N \l__knot_tmpb_tl}

  \bool_if:nTF {
    \l__knot_save_bool
    &&
    \tl_if_exist_p:c {
      knot~ intersections~
      \tl_use:N \l__knot_name_tl -
      \tl_use:N \l__knot_tmpa_tl -
      \tl_use:N \l__knot_tmpb_tl
    }
  }
  {
    \tl_use:c
    {
      knot~ intersections~ \tl_use:N \l__knot_name_tl -
      \tl_use:N \l__knot_tmpa_tl -
      \tl_use:N \l__knot_tmpb_tl
    }
  }
  {
    \pgfintersectionofpaths{\pgfsetpath\l__knot_tmpc_tl}{\pgfsetpath\l__knot_tmpd_tl}

  }

  \knot_debug:x {found~\pgfintersectionsolutions\c_space_tl~ intersections}
  \int_compare:nT {\pgfintersectionsolutions > 0}
  {
    \int_step_function:nnnN
    {1}
    {1}
    {\pgfintersectionsolutions}
    \knot_do_intersection:n
  }

  \knot_save_intersections:VV \l__knot_tmpa_tl \l__knot_tmpb_tl
  \group_end:
}
\cs_new_protected_nopar:Npn \knot_save_intersections:nn #1#2
{
  \knot_debug:n {knot~ save~ intersections}
  \bool_if:NT \l__knot_save_bool
  {
    \tl_clear:N \l__knot_aux_tl
    \tl_put_right:Nn \l__knot_aux_tl
    {
      \def\pgfintersectionsolutions
    }
    \tl_put_right:Nx \l__knot_aux_tl
    {
      {\int_eval:n {\pgfintersectionsolutions}}
    }
    \int_compare:nT {\pgfintersectionsolutions > 0}
    {
      \int_step_inline:nnnn {1} {1} {\pgfintersectionsolutions}
      {
        \pgfpointintersectionsolution{##1}
        \dim_set:Nn \l__knot_tmpa_dim {\pgf@x}
        \dim_set:Nn \l__knot_tmpb_dim {\pgf@y}
        \tl_put_right:Nn \l__knot_aux_tl
        {
          \expandafter\def\csname pgfpoint@intersect@solution@##1\endcsname
        }
        \tl_put_right:Nx \l__knot_aux_tl
        {
          {
            \exp_not:N \pgf@x
            =
            \dim_use:N \l__knot_tmpa_dim
            \exp_not:N \relax
            \exp_not:N \pgf@y
            =
            \dim_use:N \l__knot_tmpb_dim
            \exp_not:N \relax
          }
        }
      }
      \tl_set:Nn \l__knot_auxa_tl {\expandafter \gdef \csname knot~ intersections~}
      \tl_put_right:Nx \l__knot_auxa_tl {\tl_use:N \l__knot_name_tl - #1 - #2}
      \tl_put_right:Nn \l__knot_auxa_tl {\endcsname}
      \tl_put_right:Nx \l__knot_auxa_tl {{\tl_to_str:N \l__knot_aux_tl}}
      \protected@write\@auxout{}{\tl_to_str:N \l__knot_auxa_tl}
    }
  }
}
\cs_generate_variant:Nn \knot_save_intersections:nn {VV}
\cs_new_protected_nopar:Npn \knot_do_intersection:n #1
{
  \knot_debug:n {knot~ do~ intersection~ #1}
  \pgfpointintersectionsolution{#1}
  \dim_set:Nn \l__knot_tmpa_dim {\pgf@x}
  \dim_set:Nn \l__knot_tmpb_dim {\pgf@y}
  \knot_debug:x {intersection~at~
    (\dim_use:N \l__knot_tmpa_dim,\dim_use:N \l__knot_tmpb_dim)}
  \bool_set_false:N \l__knot_skip_bool
  \bool_if:NT \l__knot_self_intersections_bool
  {
    \tl_set:Nn \l__knot_tmpc_tl {knot previous}
    \tl_put_right:NV \l__knot_tmpc_tl \l__knot_tmpa_tl
    \tl_set:Nv \l__knot_tmpc_tl \l__knot_tmpc_tl
    \tl_if_eq:NNT \l__knot_tmpc_tl \l__knot_tmpb_tl
    {
      \knot_test_endpoint:NVnT \l__knot_tolerance_dim \l__knot_tmpb_tl {final point}
      {
        \bool_set_true:N \l__knot_skip_bool
      }
    }

    \tl_set:Nn \l__knot_tmpc_tl {knot previous}
    \tl_put_right:NV \l__knot_tmpc_tl \l__knot_tmpb_tl
    \tl_set:Nv \l__knot_tmpc_tl \l__knot_tmpc_tl
    \tl_if_eq:NNT \l__knot_tmpc_tl \l__knot_tmpa_tl
    {
      \knot_test_endpoint:NVnT \l__knot_tolerance_dim \l__knot_tmpa_tl {final point}
      {
        \bool_set_true:N \l__knot_skip_bool
      }
    }
  }
  \bool_if:NT \l__knot_ignore_ends_bool
  {
    \knot_test_endpoint:NVnT \l__knot_tolerance_dim \l__knot_tmpa_tl {initial point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:NVnT \l__knot_tolerance_dim \l__knot_tmpa_tl {final point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:NVnT \l__knot_tolerance_dim \l__knot_tmpb_tl {initial point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:NVnT \l__knot_tolerance_dim \l__knot_tmpb_tl {final point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
  }
  \bool_if:NF \l__knot_skip_bool
  {

    \int_gincr:N \g__knot_intersections_int
    \knot_debug:x {Processing~intersection~\int_use:N \g__knot_intersections_int}
    \bool_if:nF
    {
      \tl_if_exist_p:c {l__knot_ignore_crossing_ \int_use:N
        \g__knot_intersections_int}
      &&
      ! \tl_if_empty_p:c {l__knot_ignore_crossing_ \int_use:N
        \g__knot_intersections_int}
    }
    {
      \bool_if:nTF
      {
        \tl_if_exist_p:c {l__knot_crossing_ \int_use:N
          \g__knot_intersections_int}
        &&
        ! \tl_if_empty_p:c {l__knot_crossing_ \int_use:N
          \g__knot_intersections_int}
      }
      {
        \tl_set_eq:NN \l__knot_tmpg_tl \l__knot_tmpb_tl
      }
      {
        \tl_set_eq:NN \l__knot_tmpg_tl \l__knot_tmpa_tl
      }
      \bool_if:NT \l__knot_self_intersections_bool
      {
        \knot_test_endpoint:NVnT
        \l__knot_redraw_tolerance_dim \l__knot_tmpg_tl {initial point}
        {
          \bool_set_true:N \l__knot_prepend_prev_bool
        }
        {
          \bool_set_false:N \l__knot_prepend_prev_bool
        }
        \knot_test_endpoint:NVnT
        \l__knot_redraw_tolerance_dim \l__knot_tmpg_tl {final point}
        {
          \bool_set_true:N \l__knot_append_next_bool
        }
        {
          \bool_set_false:N \l__knot_append_next_bool
        }
        \bool_if:nT
        {
          \l__knot_prepend_prev_bool || \l__knot_append_next_bool
        }
        {
          \tl_clear_new:c {knot \tl_use:N \l__knot_prefix_tl -1}
          \tl_set_eq:cc
          {knot \tl_use:N \l__knot_prefix_tl -1}
          {knot \tl_use:N \l__knot_tmpg_tl}

          \tl_clear_new:c {l__knot_options_ \tl_use:N \l__knot_prefix_tl -1}
          \tl_set_eq:cc
          {l__knot_options_ \tl_use:N \l__knot_prefix_tl -1}
          {l__knot_options_ \tl_use:N \l__knot_tmpg_tl}

          \bool_if:nT
          {
            \l__knot_prepend_prev_bool
            &&
            \tl_if_exist_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
            &&
            !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          }
          {
            \knot_debug:x {Prepending~
              \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}}
            \spath_prepend_no_move:cv
            {knot \tl_use:N \l__knot_prefix_tl -1}
            {knot \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}}
            \bool_if:nT
            {
              \l__knot_splits_bool
              &&
              \tl_if_exist_p:c {knot previous
                \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}
              }
              &&
              !\tl_if_empty_p:c {knot previous
                \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}
              }
            }
            {
              \knot_test_endpoint:NvnT
              \l__knot_redraw_tolerance_dim
              {knot previous \tl_use:N \l__knot_tmpg_tl}
              {initial point}
              {
                \knot_debug:x {Prepending~
                  \tl_use:c {knot previous
                    \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}
                  }
                }
                \spath_prepend_no_move:cv
                {knot \tl_use:N \l__knot_prefix_tl -1}
                {knot \tl_use:c
                  {knot previous \tl_use:c
                    {knot previous \tl_use:N \l__knot_tmpg_tl}
                  }
                }
                \tl_set_eq:Nc \l__knot_tmpa_tl
                {knot \tl_use:N \l__knot_prefix_tl -1}
              }
            }
          }

          \bool_if:nT
          {
            \l__knot_append_next_bool
            &&
            \tl_if_exist_p:c {knot next \tl_use:N \l__knot_tmpg_tl}
            &&
            !\tl_if_empty_p:c {knot next \tl_use:N \l__knot_tmpg_tl}
          }
          {
            \knot_debug:x {Appending~
              \tl_use:c {knot next \tl_use:N \l__knot_tmpg_tl}}
            \spath_append_no_move:cv
            {knot \tl_use:N \l__knot_prefix_tl -1}
            {knot \tl_use:c {knot next \tl_use:N \l__knot_tmpg_tl}}
            \bool_if:nT
            {
              \l__knot_splits_bool
              &&
              \tl_if_exist_p:c {knot next \tl_use:c { knot next \tl_use:N
                \l__knot_tmpg_tl}}
              &&
              !\tl_if_empty_p:c {knot next
                \tl_use:c { knot next \tl_use:N \l__knot_tmpg_tl}
              }
            }
            {
              \knot_debug:x {Testing~ whether~ to~ append~
                {knot next \tl_use:c { knot next \tl_use:N \l__knot_tmpg_tl}}
              }
              \knot_test_endpoint:NvnT
              \l__knot_redraw_tolerance_dim
              {knot next \tl_use:N \l__knot_tmpg_tl}
              {final point}
              {
                \knot_debug:x {Appending~
                  {knot next \tl_use:c { knot next \tl_use:N \l__knot_tmpg_tl}}
                }
                \spath_append_no_move:cv
                {knot \tl_use:N \l__knot_prefix_tl -1}
                {knot \tl_use:c
                  {knot next \tl_use:c
                    {knot next \tl_use:N \l__knot_tmpg_tl}
                  }
                }
              }
            }
          }
          \tl_set:Nn \l__knot_tmpg_tl {\tl_use:N \l__knot_prefix_tl -1}
        }
      }
      \pgfscope
      \group_begin:
      \tikzset{
        knot~ diagram/every~ intersection/.try,
        every~ intersection/.try,
        knot~ diagram/intersection~ \int_use:N \g__knot_intersections_int/.try
      }
      \knot_draw_crossing:VVV \l__knot_tmpg_tl \l__knot_tmpa_dim \l__knot_tmpb_dim
      \coordinate
      (\l__knot_name_tl \c_space_tl \int_use:N \g__knot_intersections_int)
      at (\dim_use:N \l__knot_tmpa_dim, \dim_use:N \l__knot_tmpb_dim);
      \group_end:
      \endpgfscope
    }
    \tl_if_empty:NF \l__knot_node_tl
    {
      \seq_gpush:Nx
      \g__knot_nodes_seq
      {
        \l__knot_node_tl
        at
        (\dim_use:N \l__knot_tmpa_dim, \dim_use:N \l__knot_tmpb_dim) {};
      }
    }
  }
}

\cs_generate_variant:Nn \knot_intersections:nn {VV}
\prg_new_conditional:Npnn \knot_test_endpoint:NN #1#2 {p,T,F,TF}
{
  \dim_compare:nTF
  {
    \dim_abs:n { \l__knot_tmpa_dim - \tl_item:Nn #2 {1}}
    +
    \dim_abs:n { \l__knot_tmpb_dim - \tl_item:Nn #2 {2}}
    <
    #1
  }
  {
    \prg_return_true:
  }
  {
    \prg_return_false:
  }
}
\prg_new_protected_conditional:Npnn \knot_test_endpoint:Nnn #1#2#3 {T,F,TF}
{
  \use:c {spath_#3:Nv} \l__knot_tmpd_tl {knot #2}
  \knot_test_endpoint:NNTF #1 \l__knot_tmpd_tl
  {
    \prg_return_true:
  }
  {
    \prg_return_false:
  }
}

\cs_generate_variant:Nn \knot_test_endpoint:NnnT {NVnT,NvnT}
\cs_generate_variant:Nn \knot_test_endpoint:NnnF {NVnF,NvnF}
\cs_generate_variant:Nn \knot_test_endpoint:NnnTF {NVnTF,NvnTF}
\cs_new_protected_nopar:Npn \knot_draw_crossing:nnn #1#2#3
{
  \knot_debug:n {knot~ draw~ crossing}
  \group_begin:
  \pgfscope
  \path[knot~ diagram/background~ clip] (#2, #3)
  circle[radius=\l__knot_clip_bg_radius_dim];

  \tl_set:Nn \l__knot_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_if_exist:cT {l__knot_options_ #1}
  {
  \tl_put_right:Nv \l__knot_tmpa_tl {l__knot_options_ #1}
  }
  \tl_put_right:Nn \l__knot_tmpa_tl
  {
    ,knotbg
    ,line~ width= \tl_use:N \l__knot_clip_width_tl * \pgflinewidth
  }
  \spath_tikz_path:Vv \l__knot_tmpa_tl {knot #1}

  \endpgfscope

  \pgfscope
  \path[knot~ diagram/clip] (#2, #3)
  circle[radius=\l__knot_clip_draw_radius_dim];

  \tl_set:Nn \l__knot_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_if_exist:cT {l__knot_options_ #1}
  {
  \tl_put_right:Nv \l__knot_tmpa_tl {l__knot_options_ #1}
  }
  \tl_put_right:Nn \l__knot_tmpa_tl
  {
    ,knot~ diagram/only~ when~ rendering/.try
    ,only~ when~ rendering/.try
  }
  \spath_tikz_path:Vv \l__knot_tmpa_tl {knot #1}

  \endpgfscope
  \group_end:
}

\cs_generate_variant:Nn \knot_draw_crossing:nnn {nVV, VVV}

\cs_new_protected_nopar:Npn \knot_draw_crossing:nn #1#2
{
  \tikz@scan@one@point\pgfutil@firstofone #2 \relax
  \knot_draw_crossing:nVV {#1} \pgf@x \pgf@y
}
\cs_new_protected_nopar:Npn \knot_split_strands:
{
  \knot_debug:n {knot~ split~ strands}
  \int_gzero:N \g__knot_filaments_int
  \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_split_strand:n
  \int_step_function:nnnN {1} {1} {\g__knot_filaments_int} \knot_compute_nexts:n
}
\cs_new_protected_nopar:Npn \knot_compute_nexts:n #1
{
  \knot_debug:n {knot~ compute~ nexts}
  \tl_clear_new:c {knot next \tl_use:c {knot previous filament #1}}
  \tl_set:cn {knot next \tl_use:c {knot previous filament #1}} {filament #1}
}
\cs_new_protected_nopar:Npn \knot_split_strand:n #1
{
  \knot_debug:n {knot~ split~ strand}
  \int_set_eq:NN \l__knot_component_start_int \g__knot_filaments_int
  \int_incr:N \l__knot_component_start_int
  \tl_set_eq:Nc \l__knot_tmpa_tl {l__knot_options_strand #1}
  \spath_segments_to_seq:Nv \l__knot_segments_seq {knot strand #1}
  \seq_map_function:NN \l__knot_segments_seq \knot_save_filament:N
}
\cs_new_protected_nopar:Npn \knot_save_filament:N #1
{
  \knot_debug:n {knot~ save~ filament}
  \tl_set:Nx \l__knot_tmpb_tl {\tl_item:nn {#1} {4}}
  \tl_case:NnF \l__knot_tmpb_tl
  {
    \c_spath_moveto_tl
    {
      \int_compare:nT {\l__knot_component_start_int < \g__knot_filaments_int}
      {
        \int_set_eq:NN \l__knot_component_start_int \g__knot_filaments_int
      }
    }
    \c_spath_lineto_tl
    {
      \int_gincr:N \g__knot_filaments_int
      \tl_clear_new:c {knot filament \int_use:N \g__knot_filaments_int}
      \tl_set:cn {knot filament \int_use:N \g__knot_filaments_int} {#1}

      \tl_clear_new:c {l__knot_options_filament \int_use:N \g__knot_filaments_int}
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \g__knot_filaments_int}
      \l__knot_tmpa_tl

      \tl_clear_new:c {knot previous filament \int_use:N \g__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \g__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \g__knot_filaments_int}
        {filament \int_eval:n {\g__knot_filaments_int - 1}}
      }
    }
    \c_spath_curvetoa_tl
    {
      \int_gincr:N \g__knot_filaments_int
      \tl_clear_new:c {knot filament \int_use:N \g__knot_filaments_int}
      \tl_set:cn {knot filament \int_use:N \g__knot_filaments_int} {#1}
      \tl_clear_new:c {l__knot_options_filament \int_use:N \g__knot_filaments_int}
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \g__knot_filaments_int}
      \l__knot_tmpa_tl

      \tl_clear_new:c {knot previous filament \int_use:N \g__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \g__knot_filaments_int}
      {
        \tl_set:cx
        {knot previous filament \int_use:N \g__knot_filaments_int}
        {filament \int_eval:n {\g__knot_filaments_int - 1}}
      }
    }
    \c_spath_closepath_tl
    {
      \int_gincr:N \g__knot_filaments_int
      \tl_clear_new:c {knot filament \int_use:N \g__knot_filaments_int}
      \tl_clear:N \l__knot_tmpa_tl
      \tl_put_right:Nx
      {
        \tl_item:nn {#1} {1}\tl_item:nn {#1} {2}\tl_item:nn {#1} {3}
      }
      \tl_put_right:NV \l__knot_tmpa_tl \c_spath_lineto_tl
      \tl_put_right:Nx {\tl_item:nn {#1} {5}\tl_item:nn {#1} {6}}

      \tl_set:cV {knot filament \int_use:N \g__knot_filaments_int} \l__knot_tmpa_tl
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \g__knot_filaments_int}
      \l__knot_tmpa_tl
      \tl_clear_new:c {knot previous filament \int_use:N \g__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \g__knot_filaments_int}
      {
        \tl_set:cx
        {knot previous filament \int_use:N \g__knot_filaments_int}
        {filament \int_eval:n {\g__knot_filaments_int - 1}}
      }
      \tl_set:cx
      {knot previous filament \int_use:N \l__knot_component_start_int}
      {filament \int_use:N \g__knot_filaments_int}
    }
  }
  {
  }
}
\NewDocumentCommand \redraw { m m }
{
  \tl_put_right:Nn \l__knot_redraws_tl {\knot_draw_crossing:nn}
  \tl_put_right:Nx \l__knot_redraws_tl {
    {strand #1} {#2}% {\dim_use:N \pgf@x} {\dim_use:N \pgf@y}
  }
}
\ExplSyntaxOff
\def\pgf@sh@@knotanchor#1#2{%
  \anchor{#2 north west}{%
    \csname pgf@anchor@knot #1@north west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 north east}{%
    \csname pgf@anchor@knot #1@north east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south west}{%
    \csname pgf@anchor@knot #1@south west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south east}{%
    \csname pgf@anchor@knot #1@south east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 north}{%
    \csname pgf@anchor@knot #1@north\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 east}{%
    \csname pgf@anchor@knot #1@east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 west}{%
    \csname pgf@anchor@knot #1@west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south}{%
    \csname pgf@anchor@knot #1@south\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
}
\pgfdeclareshape{knot crossing}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritanchorborder[from=circle]
  \pgf@sh@@knotanchor{crossing}{2}
  \pgf@sh@@knotanchor{crossing}{3}
  \pgf@sh@@knotanchor{crossing}{4}
  \pgf@sh@@knotanchor{crossing}{8}
  \pgf@sh@@knotanchor{crossing}{16}
  \pgf@sh@@knotanchor{crossing}{32}
  \backgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
  }
}
\pgfdeclareshape{knot over cross}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
  }
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}
\pgfdeclareshape{knot under cross}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
  }
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
 }
}
\pgfdeclareshape{knot vert}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}
\pgfdeclareshape{knot horiz}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
 }
}
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  spath3_code.dtx
%%                                  calligraphy_doc.tex
%%                                  knots_doc.tex
%%                                  spath3.tex
%% and the derived files            spath3.ins,
%%                                  spath3_code.pdf,
%%                                  spath3.sty,
%%                                  tikzlibrarycalligraphy.code.tex
%%                                  tikzlibraryknots.code.tex
%%                                  tikzlibraryspath3.code.tex
%%                                  calligraphy.pdf
%%                                  knots.pdf
%%                                  spath3.pdf
%%                                  README
%% 
%%
%% End of file `tikzlibraryknots.code.tex'.


==> tikzlibraryspath3.code.tex <==
%%
%% This is file `tikzlibraryspath3.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% spath3-code.dtx  (with options: `tikzspath3')
%% ----------------------------------------------------------------
%% spath3 --- Functions for manipulating PGF soft paths
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\RequirePackage{spath3}
\RequirePackage{expl3}
\ExplSyntaxOn

\tl_new:N \l__tikzspath_tmpa_tl
\tl_new:N \l__tikzspath_tmpb_tl
\tl_new:N \l__tikzspath_tmpc_tl
\tl_new:N \l__tikzspath_tmpd_tl
\tl_new:N \l__tikzspath_tmpe_tl
\tl_new:N \l__tikzspath_tmpf_tl

\int_new:N \l__tikzspath_tmpa_int
\seq_new:N \l__tikzspath_tmpa_seq
\seq_new:N \l__tikzspath_tmpb_seq
\seq_new:N \l__tikzspath_tmpc_seq
\seq_new:N \l__tikzspath_tmpd_seq

\tl_new:N \l__tikzspath_current_tl
\tl_new:N \l__tikzspath_reverse_tl
\tl_new:N \l__tikzspath_prefix_tl
\tl_new:N \l__tikzspath_suffix_tl
\tl_new:N \g__tikzspath_smuggle_tl
\tl_new:N \g__tikzspath_output_tl
\tl_new:N \l__tikzspath_check_tl
\clist_new:N \g__tikzspath_output_clist
\seq_new:N \g__tikzspath_tmpa_seq
\seq_new:N \g__tikzspath_tmpb_seq
\seq_new:N \g__tikzspath_output_seq
\bool_new:N \l__tikzspath_draft_bool
\msg_new:nnn { spath3 } { missing soft path }
{ Soft~ path~ #1~ doesn't~ exist~ \msg_line_context:}
\msg_new:nnnn { spath3 } { empty soft path }
{ Soft~ path~ #1~ is~ empty~ \msg_line_context:}
{If~ it~ was~ defined~ inside~ a~ group,~ try~ using~ "save~ global". }
\msg_new:nnn { spath3 } { load intersections }
{ You~ need~ to~ load~ the~ "intersections"~ library~
  to~ work~ with~ intersections }
\tl_set:Nn \l__tikzspath_prefix_tl {tikz@intersect@path@name@}
\tl_set:Nn \l__tikzspath_suffix_tl {}
\tl_new:N \g__tikzspath_tikzfinish_tl
\tl_new:N \l__tikzspath_tikzfinish_outside_tl
\cs_new_protected_nopar:Npn \spath_at_end_of_path:
{
  \tl_use:N \g__tikzspath_tikzfinish_tl
  \tl_gclear:N \g__tikzspath_tikzfinish_tl
}
\tl_put_right:Nn \tikz@finish {\spath_at_end_of_path:}

\tikzset{
  every~ scope/.append~ style={
    execute~ at~ begin~ scope={
      \tl_set_eq:NN \l__tikzspath_tikzfinish_outside_tl \g__tikzspath_tikzfinish_tl
    },
    execute~ at~ end~ scope={
      \tl_use:N \g__tikzspath_tikzfinish_tl
      \tl_gclear:N \g__tikzspath_tikzfinish_tl
      \tl_gset_eq:NN \g__tikzspath_tikzfinish_tl \l__tikzspath_tikzfinish_outside_tl
    },
  },
}
\tl_new:N \l__tikzspath_tikzpath_finish_tl

\cs_new_protected_nopar:Npn \__tikzspath_at_end_of_path_construction:
{
  \tl_use:N \l__tikzspath_tikzpath_finish_tl
  \tl_clear:N \l__tikzspath_tikzpath_finish_tl
}

\tl_put_left:Nn \tikz@finish {\__tikzspath_at_end_of_path_construction:}
\cs_new_protected_nopar:Npn \spath_save_path:Nn #1#2
{
  \tl_if_empty:NF \g__tikzspath_tikzfinish_tl
  {
    \tl_use:N \g__tikzspath_tikzfinish_tl
  }
  \tl_gput_right:Nn \g__tikzspath_tikzfinish_tl
  {
    \tl_clear_new:N #1
    \tl_set:Nn #1 {#2}
  }
}
\cs_generate_variant:Nn \spath_save_path:Nn {cn, NV, cV}

\cs_new_protected_nopar:Npn \spath_gsave_path:Nn #1#2
{
  \tl_gput_right:Nn \g__tikzspath_tikzfinish_tl
  {
    \tl_gclear_new:N #1
    \tl_gset:Nn #1 {#2}
  }
}
\cs_generate_variant:Nn \spath_gsave_path:Nn {cn, NV, cV}
\cs_new_protected_nopar:Npn \__tikzspath_process_tikz_point:Nn #1#2
{
  \group_begin:
  \use:c {tikz@scan@one@point} \use:n #2 \scan_stop:
  \tl_gset:Nx \g__tikzspath_output_tl
  {
    { \dim_use:c {pgf@x} }
    { \dim_use:c {pgf@y} }
  }
  \group_end:
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_set_eq:NN \__tikzspath_tikzset:n \tikzset
\cs_generate_variant:Nn \__tikzspath_tikzset:n {V, v}
\cs_new_protected_nopar:Npn \__tikzspath_check_path:nnn #1#2#3
{
  \tl_set:Nn \l__tikzspath_check_tl {#3}
  \tl_if_exist:cTF {\__tikzspath_path_name:n {#2}}
  {
    \tl_if_empty:cTF {\__tikzspath_path_name:n {#2}}
    {
      \msg_warning:nnn { spath3 } { empty soft path } { #2 }
    }
    {
      \tl_set:Nn \l__tikzspath_check_tl {
        #1 {\__tikzspath_path_name:n {#2}}
      }
    }
  }
  {
    \msg_warning:nnn { spath3 } { missing soft path } { #2 }
  }
  \tl_use:N \l__tikzspath_check_tl
}
\cs_new_protected_nopar:Npn \__tikzspath_check_two_paths:nnnn #1#2#3#4
{
  \__tikzspath_check_path:nnn {
    \__tikzspath_check_path:nnn {#1}{#2}{#4}
  }{#3}{#4}
}
\cs_new_protected_nopar:Npn \__tikzspath_check_three_paths:nnnnn #1#2#3#4#5
{
  \__tikzspath_check_path:nnn {
    \__tikzspath_check_path:nnn {
      \__tikzspath_check_path:nnn {#1}{#2}{#5}
    }{#3}{#5}
  }{#4}{#5}
}
\cs_generate_variant:Nn \__tikzspath_check_path:nnn {nVn}
\cs_generate_variant:Nn \__tikzspath_check_two_paths:nnnn {nnVn}
\cs_new_protected_nopar:Npn \__tikzspath_maybe_current_path:nn #1#2
{
  \tl_if_eq:nnT {#2} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#2}}
  }
  #1 {#2}
}
\cs_new_protected_nopar:Npn \__tikzspath_maybe_current_path_reuse:nnn #1#2#3
{
  \bool_set_true:N \l_spath_movetorelevant_bool
  \tl_if_eq:nnT {#2} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#2}}
  }
  #1 {#2} #3
  \tl_if_eq:nnT {#2} {current}
  {
    \tl_if_empty:cF {\__tikzspath_path_name:n {#2}}
    {
      \spath_set_current_path:c {\__tikzspath_path_name:n {#2}}
      \spath_set_tikz_data:v {\__tikzspath_path_name:n {#2}}
    }
  }
}
\cs_new_protected_nopar:Npn \__tikzspath_maybe_current_two_paths_reuse_both:nnnn #1#2#3#4
{
  \bool_set_true:N \l_spath_movetorelevant_bool
  \tl_if_eq:nnT {#2} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#2}}
  }
  \tl_if_eq:nnT {#3} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#3}}
  }
  #1 {#2} {#3} #4
  \tl_if_eq:nnT {#2} {current}
  {
    \tl_if_empty:cF {\__tikzspath_path_name:n {#2}}
    {
      \spath_set_current_path:c {\__tikzspath_path_name:n {#2}}
      \spath_set_tikz_data:v {\__tikzspath_path_name:n {#2}}
    }
  }
  \tl_if_eq:nnT {#3} {current}
  {
    \tl_if_empty:cF {\__tikzspath_path_name:n {#3}}
    {
      \spath_set_current_path:c {\__tikzspath_path_name:n {#3}}
      \spath_set_tikz_data:v {\__tikzspath_path_name:n {#3}}
    }
  }
}
\cs_new_protected_nopar:Npn \__tikzspath_maybe_current_two_paths_reuse_first:nnnn #1#2#3#4
{
  \bool_set_true:N \l_spath_movetorelevant_bool
  \tl_if_eq:nnT {#2} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#2}}
  }
  \tl_if_eq:nnT {#3} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#3}}
  }
  #1 {#2} {#3} #4
  \tl_if_eq:nnT {#2} {current}
  {
    \tl_if_empty:cF {\__tikzspath_path_name:n {#2}}
    {
      \spath_set_current_path:c {\__tikzspath_path_name:n {#2}}
      \spath_set_tikz_data:v {\__tikzspath_path_name:n {#2}}
    }
  }
}
\cs_new_protected_nopar:Npn \__tikzspath_maybe_current_two_paths_reuse_second:nnnn #1#2#3#4
{
  \bool_set_true:N \l_spath_movetorelevant_bool
  \tl_if_eq:nnT {#2} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#2}}
  }
  \tl_if_eq:nnT {#3} {current}
  {
    \spath_get_current_path:c {\__tikzspath_path_name:n {#3}}
  }
  #1 {#2} {#3} #4
  \tl_if_eq:nnT {#3} {current}
  {
    \tl_if_empty:cF {\__tikzspath_path_name:n {#3}}
    {
      \spath_set_current_path:c {\__tikzspath_path_name:n {#3}}
      \spath_set_tikz_data:v {\__tikzspath_path_name:n {#3}}
    }
  }
}
\cs_generate_variant:Nn \__tikzspath_maybe_current_path:nn {nV}
\cs_generate_variant:Nn \__tikzspath_maybe_current_path_reuse:nnn {nVn}
\cs_new_protected_nopar:Npn \__tikzspath_seq_from_foreach:Nnn #1#2#3
{
  \group_begin:
  \seq_gclear:N \g__tikzspath_output_seq

  \tl_if_empty:nTF {#3}
  {
    \int_step_inline:nnnn {1}{1} {#2}
    {
      \seq_gput_right:Nn \g__tikzspath_output_seq {##1}
    }
  }
  {
    \foreach \l__tikzspath_tmpa_tl in {#3}
    {
      \int_compare:nTF { \l__tikzspath_tmpa_tl > 0 }
      {
        \seq_gput_right:NV \g__tikzspath_output_seq \l__tikzspath_tmpa_tl
      }
      {
        \seq_gput_right:Nx \g__tikzspath_output_seq
        {\int_eval:n {#2 - \l__tikzspath_tmpa_tl}}
      }
    }
    \seq_gsort:Nn \g__tikzspath_output_seq
    {
      \int_compare:nNnTF {##1} < {##2}
      { \sort_return_same: }
      { \sort_return_swapped: }
    }
  }
  \group_end:
  \seq_set_eq:NN #1 \g__tikzspath_output_seq
  \seq_gclear:N \g__tikzspath_output_seq
}
\cs_generate_variant:Nn \__tikzspath_seq_from_foreach:Nnn {NVV, NVn}
\cs_new:Npn \__tikzspath_path_name:n #1
{
  \tl_use:N \l__tikzspath_prefix_tl
  #1
  \tl_use:N \l__tikzspath_suffix_tl
}
\cs_generate_variant:Nn \__tikzspath_path_name:n {V}
\bool_new:N \l__tikzspath_reverse_bool
\bool_new:N \l__tikzspath_weld_bool
\bool_new:N \l__tikzspath_move_bool
\bool_new:N \l__tikzspath_global_bool
\bool_new:N \l__tikzspath_current_transformation_bool
\tl_new:N \l__tikzspath_joinpath_tl
\tl_new:N \l__tikzspath_transformation_tl

\cs_new_protected_nopar:Npn \__tikzspath_set_bool:Nn #1#2
{
  \tl_if_eq:nnTF {#2}{false}
  {
    \bool_set_false:N #1
  }
  {
    \bool_set_true:N #1
  }
}
\tikzset {
  spath/join/.is~ family,
  spath/join/.cd,
  reverse/.code = {
    \__tikzspath_set_bool:Nn \l__tikzspath_reverse_bool {#1}
  },
  reverse/.default = true,
  weld/.code = {
    \__tikzspath_set_bool:Nn \l__tikzspath_weld_bool {#1}
  },
  weld/.default = true,
  no~ weld/.code = {
    \__tikzspath_set_bool:Nn \l__tikzspath_weld_bool {#1}
    \bool_set:Nn \l__tikzspath_weld_bool {! \l__tikzspath_weld_bool}
  },
  no~ weld/.default = true,
  move/.code = {
    \__tikzspath_set_bool:Nn \l__tikzspath_move_bool {#1}
  },
  move/.default = true,
  no~ move/.code = {
    \__tikzspath_set_bool:Nn \l__tikzspath_move_bool {#1}
    \bool_set:Nn \l__tikzspath_move_bool {! \l__tikzspath_move_bool}
  },
  no~ move/.default = true,
  global/.code = {
    \__tikzspath_set_bool:Nn \l__tikzspath_global_bool {#1}
  },
  global/.default = true,
  use~ current~ transformation/.code={
    \__tikzspath_set_bool:Nn \l__tikzspath_current_transformation_bool {#1}
  },
  use~ current~ transformation/.default = true,
  transform/.store~in=\l__tikzspath_transformation_tl,
  .unknown/.code = {
    \tl_set_eq:NN \l__tikzspath_joinpath_tl \pgfkeyscurrentname
  }
}
\cs_set_eq:NN \getComponentOf \clist_item:Nn
\cs_new_protected_nopar:Npn \__tikzspath_use_path:n #1
{
  \tl_set:Nn \l__tikzspath_joinpath_tl {#1}
  \spath_get_current_path:N \l__tikzspath_current_tl

  \bool_if:NT \l__tikzspath_reverse_bool
  {
    \spath_reverse:N \l__tikzspath_joinpath_tl
  }

  \bool_if:NT \l__tikzspath_current_transformation_bool
  {
    \pgfgettransform \l__tikzspath_tmpa_tl
    \spath_transform:NV
    \l__tikzspath_joinpath_tl
    \l__tikzspath_tmpa_tl
  }

  \tl_if_empty:NF \l__tikzspath_transformation_tl
  {
    \group_begin:
    \pgftransformreset
    \__tikzspath_tikzset:V \l__tikzspath_transformation_tl
    \pgfgettransform \l__tikzspath_tmpa_tl
    \tl_gset:Nn \g__tikzspath_smuggle_tl
    {
      \spath_transform:Nnnnnnn
      \l__tikzspath_joinpath_tl
    }
    \tl_gput_right:NV \g__tikzspath_smuggle_tl \l__tikzspath_tmpa_tl
    \group_end:
    \tl_use:N \g__tikzspath_smuggle_tl
  }

  \bool_if:NT \l__tikzspath_move_bool
  {
    \tl_if_empty:NTF \l__tikzspath_current_tl
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl { {0pt} {0pt} }
    }
    {
      \spath_finalpoint:NV
      \l__tikzspath_tmpc_tl
      \l__tikzspath_current_tl
    }
    \spath_translate_to:NV \l__tikzspath_joinpath_tl \l__tikzspath_tmpc_tl
  }

  \tl_if_empty:NTF \l__tikzspath_current_tl
  {
    \tl_if_empty:NTF \l__tikzspath_joinpath_tl
    {
      \tl_set_eq:NN \l__tikzspath_current_tl \c_spath_moveto_tl
      \tl_put_right:Nn \l__tikzspath_current_tl {{0pt}{0pt}}
    }
    {
      \tl_set_eq:NN \l__tikzspath_current_tl \l__tikzspath_joinpath_tl
    }
  }
  {

    \tl_clear:N \l__tikzspath_tmpa_tl
    \tl_set:Nn \l__tikzspath_tmpa_tl {spath_}

    \tl_put_right:Nn \l__tikzspath_tmpa_tl {append}

    \bool_if:NT \l__tikzspath_weld_bool
    {
      \tl_put_right:Nn \l__tikzspath_tmpa_tl {_no_move}
      \spath_numberofcomponents:NV \l__tikzspath_tmpa_int \l__tikzspath_joinpath_tl
      \int_compare:nT {\l__tikzspath_tmpa_int == 1}
      {
        \bool_set_false:N \l_spath_movetorelevant_bool
      }
    }
    \tl_put_right:Nn \l__tikzspath_tmpa_tl {:NV}

    \use:c {\tl_use:N \l__tikzspath_tmpa_tl }
    \l__tikzspath_current_tl
    \l__tikzspath_joinpath_tl
  }

  \spath_set_current_path:N \l__tikzspath_current_tl
  \spath_set_tikz_data:V \l__tikzspath_joinpath_tl
}
\cs_generate_variant:Nn \__tikzspath_use_path:n {V, v}
\cs_new_protected_nopar:Npn \__tikzspath_join_with:Nn #1#2
{
  \tl_set:Nn \l__tikzspath_joinpath_tl {#2}

  \bool_if:NT \l__tikzspath_reverse_bool
  {
    \spath_reverse:N \l__tikzspath_joinpath_tl
  }

  \tl_if_empty:NF \l__tikzspath_transformation_tl
  {
    \group_begin:
    \pgftransformreset
    \__tikzspath_tikzset:V \l__tikzspath_transformation_tl
    \pgfgettransform \l__tikzspath_tmpa_tl
    \tl_gset:Nn \g__tikzspath_smuggle_tl
    {
      \spath_transform:Nnnnnnn
      \l__tikzspath_joinpath_tl
    }
    \tl_gput_right:NV \g__tikzspath_smuggle_tl \l__tikzspath_tmpa_tl
    \group_end:
    \tl_use:N \g__tikzspath_smuggle_tl
  }

  \bool_if:NT \l__tikzspath_move_bool
  {
    \spath_finalpoint:NV
    \l__tikzspath_tmpc_tl
    #1
    \spath_translate_to:NV \l__tikzspath_joinpath_tl \l__tikzspath_tmpc_tl
  }

  \tl_clear:N \l__tikzspath_tmpa_tl
  \tl_set:Nn \l__tikzspath_tmpa_tl {spath_}

  \bool_if:NT \l__tikzspath_global_bool
  {
    \tl_put_right:Nn \l__tikzspath_tmpa_tl {g}
  }

  \tl_put_right:Nn \l__tikzspath_tmpa_tl {append}

  \bool_if:NT \l__tikzspath_weld_bool
  {
    \tl_put_right:Nn \l__tikzspath_tmpa_tl {_no_move}
  }
  \tl_put_right:Nn \l__tikzspath_tmpa_tl {:NV}

  \cs_if_exist:cF {\tl_use:N \l__tikzspath_tmpa_tl}
  {
    \tl_show:N \l__tikzspath_tmpa_tl
  }

  \use:c {\tl_use:N \l__tikzspath_tmpa_tl } #1
  \l__tikzspath_joinpath_tl
}
\cs_generate_variant:Nn \__tikzspath_join_with:Nn {cv, cn}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_with_aux:nnn #1#2#3
{
  \group_begin:
  \tl_set:Nn \l__tikzspath_tmpc_tl {#1}
  \tl_if_empty:nT {#3}
  {
    \spath_spot_weld_components:N \l__tikzspath_tmpc_tl
  }

  \spath_numberofcomponents:NV \l__tikzspath_tmpa_int \l__tikzspath_tmpc_tl
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpb_seq \l__tikzspath_tmpa_int {#3}

  \spath_components_to_seq:NV \l__tikzspath_tmpa_seq \l__tikzspath_tmpc_tl

  \seq_pop_left:NN \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_tl
  \seq_pop_left:NN \l__tikzspath_tmpb_seq \l__tikzspath_tmpb_tl

  \seq_map_indexed_inline:Nn \l__tikzspath_tmpa_seq
  {
    \int_compare:nTF
    {
      ##1 == \l__tikzspath_tmpb_tl
    }
    {
      \seq_pop_left:NNF \l__tikzspath_tmpb_seq \l__tikzspath_tmpb_tl
      {
        \tl_set:Nn \l__tikzspath_tmpb_tl {-1}
      }
      \spath_splice_between:Nnn \l__tikzspath_tmpa_tl {#2} {##2}
    }
    {
      \tl_put_right:Nn \l__tikzspath_tmpa_tl {##2}
    }
  }
  \tl_gset_eq:NN \g__tikzspath_output_tl \l__tikzspath_tmpa_tl
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_with:Nnnn #1#2#3#4
{
  \__tikzspath_join_components_with_aux:nnn {#2}{#3}{#4}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_join_components_with:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_with:Nnn #1#2#3
{
  \__tikzspath_join_components_with:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_join_components_with:Nnn {cvV}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components_with:Nnnn #1#2#3#4
{
  \__tikzspath_join_components_with_aux:nnn {#2}{#3}{#4}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components_with:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components_with:Nnn #1#2#3
{
  \__tikzspath_gjoin_components_with:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components_with:Nnn {cvV}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_upright_with_aux:nnn #1#2#3
{
  \group_begin:
  \tl_set:Nn \l__tikzspath_tmpc_tl {#1}
  \tl_if_empty:nT {#3}
  {
    \spath_spot_weld_components:N \l__tikzspath_tmpc_tl
  }

  \spath_numberofcomponents:NV \l__tikzspath_tmpa_int \l__tikzspath_tmpc_tl
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpb_seq \l__tikzspath_tmpa_int {#3}

  \spath_components_to_seq:NV \l__tikzspath_tmpa_seq \l__tikzspath_tmpc_tl

  \seq_pop_left:NN \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_tl
  \seq_pop_left:NN \l__tikzspath_tmpb_seq \l__tikzspath_tmpb_tl

  \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
  \spath_transform:NVnnnnnn \l__tikzspath_tmpd_tl \l__tikzspath_tmpc_tl {1}{0}{0}{-1}{0pt}{0pt}

  \seq_map_indexed_inline:Nn \l__tikzspath_tmpa_seq
  {
    \int_compare:nTF
    {
      ##1 == \l__tikzspath_tmpb_tl
    }
    {
      \seq_pop_left:NNF \l__tikzspath_tmpb_seq \l__tikzspath_tmpb_tl
      {
        \tl_set:Nn \l__tikzspath_tmpb_tl {-1}
      }

      \spath_finalpoint:NV \l__tikzspath_tmpe_tl \l__tikzspath_tmpa_tl
      \spath_initialpoint:Nn \l__tikzspath_tmpf_tl {##2}

      \dim_compare:nTF
      {
        \tl_item:Nn \l__tikzspath_tmpe_tl {1}
        >
        \tl_item:Nn \l__tikzspath_tmpf_tl {1}
      }
      {
        \spath_splice_between:NVn
        \l__tikzspath_tmpa_tl
        \l__tikzspath_tmpd_tl
        {##2}
      }
      {
        \spath_splice_between:NVn
        \l__tikzspath_tmpa_tl
        \l__tikzspath_tmpc_tl
        {##2}
      }
    }
    {
      \tl_put_right:Nn \l__tikzspath_tmpa_tl {##2}
    }
  }
  \tl_gset_eq:NN \g__tikzspath_output_tl \l__tikzspath_tmpa_tl
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_upright_with:Nnnn #1#2#3#4
{
  \__tikzspath_join_components_upright_with_aux:nnn {#2}{#3}{#4}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_join_components_upright_with:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_upright_with:Nnn #1#2#3
{
  \__tikzspath_join_components_upright_with:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_join_components_upright_with:Nnn {cvV}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components_upright_with:Nnnn #1#2#3#4
{
  \__tikzspath_join_components_upright_with_aux:nnn {#2}{#3}{#4}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components_upright_with:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components_upright_with:Nnn #1#2#3
{
  \__tikzspath_gjoin_components_upright_with:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components_upright_with:Nnn {cvV}
\cs_new_protected_nopar:Npn \__tikzspath_get_components_aux:n #1
{
  \clist_gclear_new:N \g__tikzspath_output_clist
  \spath_components_to_seq:Nn \l__tikzspath_tmpa_seq {#1}

  \seq_map_inline:Nn \l__tikzspath_tmpa_seq
  {
    \spath_anonymous:N \l__tikzspath_tmpa_tl
    \tl_new:c {\__tikzspath_path_name:V \l__tikzspath_tmpa_tl}
    \tl_set:cn {\__tikzspath_path_name:V \l__tikzspath_tmpa_tl} {##1}
    \clist_gput_right:NV \g__tikzspath_output_clist \l__tikzspath_tmpa_tl
  }
}
\cs_new_protected_nopar:Npn \__tikzspath_get_components:Nn #1#2
{
  \clist_clear_new:N #1
  \__tikzspath_get_components_aux:n {#2}
  \clist_set_eq:NN #1 \g__tikzspath_output_clist
  \clist_gclear:N \g__tikzspath_output_clist
}
\cs_generate_variant:Nn \__tikzspath_get_components:Nn {NV, Nv}
\cs_new_protected_nopar:Npn \__tikzspath_gget_components:Nn #1#2
{
  \clist_gclear_new:N #1
  \__tikzspath_get_components_aux:n {#2}
  \clist_gset_eq:NN #1 \g__tikzspath_output_clist
  \clist_gclear:N \g__tikzspath_output_clist
}
\cs_generate_variant:Nn \__tikzspath_gget_components:Nn {NV, Nv}
\cs_new_protected_nopar:Npn \__tikzspath_render_components:nn #1#2
{
  \group_begin:
  \spath_components_to_seq:Nn \l__tikzspath_tmpa_seq {#2}
  \seq_map_indexed_inline:Nn \l__tikzspath_tmpa_seq
  {
    \spath_tikz_path:nn
    {
      every~ spath~ component/.try,
      spath ~component~ ##1/.try,
      spath ~component/.try={##1},
      every~ #1~ component/.try,
      #1 ~component~ ##1/.try,
      #1 ~component/.try={##1},
    }
    {
      ##2
    }
  }
  \group_end:
}
\cs_generate_variant:Nn \__tikzspath_render_components:nn {nv}
\cs_new_protected_nopar:Npn \__tikzspath_insert_gaps_after_components_aux:nnn #1#2#3
{
  \group_begin:
  \spath_numberofcomponents:Nn \l__tikzspath_tmpa_int {#1}
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_int {#3}

  \tl_if_empty:nT {#3}
  {
    \seq_pop_right:NN \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_tl
  }

  \seq_clear:N \l__tikzspath_tmpb_seq
  \seq_map_inline:Nn \l__tikzspath_tmpa_seq {
    \seq_put_right:Nx
    \l__tikzspath_tmpb_seq
    {\int_eval:n
      {
        \int_mod:nn { ##1 }{ \l__tikzspath_tmpa_int } + 1
      }
    }
  }

  \spath_components_to_seq:Nn \l__tikzspath_tmpc_seq {#1}

  \seq_clear:N \l__tikzspath_tmpd_seq
  \seq_map_indexed_inline:Nn \l__tikzspath_tmpc_seq
  {
    \tl_set:Nn \l__tikzspath_tmpa_tl {##2}
    \seq_if_in:NnT \l__tikzspath_tmpa_seq {##1}
    {
      \spath_shorten_at_end:Nn \l__tikzspath_tmpa_tl {(#2)/2}
    }
    \seq_if_in:NnT \l__tikzspath_tmpb_seq {##1}
    {
      \spath_shorten_at_start:Nn \l__tikzspath_tmpa_tl {(#2)/2}
    }
    \seq_put_right:NV \l__tikzspath_tmpd_seq \l__tikzspath_tmpa_tl
  }
  \tl_gset:Nx \g__tikzspath_output_tl {\seq_use:Nn \l__tikzspath_tmpd_seq {} }
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_insert_gaps_after_components:Nnnn #1#2#3#4
{
  \__tikzspath_insert_gaps_after_components_aux:nnn {#2}{#3}{#4}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_insert_gaps_after_components:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_insert_gaps_after_components:Nnn #1#2#3
{
  \__tikzspath_insert_gaps_after_components:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_insert_gaps_after_components:Nnn {cnn, cVV}
\cs_new_protected_nopar:Npn \__tikzspath_ginsert_gaps_after_components:Nnnn #1#2#3#4
{
  \__tikzspath_insert_gaps_after_components_aux:nnn {#2}{#3}{#4}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_ginsert_gaps_after_components:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_ginsert_gaps_after_components:Nnn #1#2#3
{
  \__tikzspath_ginsert_gaps_after_components:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_ginsert_gaps_after_components:Nnn {cnn, cVV}
\cs_new_protected_nopar:Npn \__tikzspath_insert_gaps_after_segments_aux:nnn #1#2#3
{
  \group_begin:
  \spath_reallength:Nn \l__tikzspath_tmpa_int {#1}
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_int {#3}

  \tl_if_empty:nT {#3}
  {
    \seq_pop_right:NN \l__tikzspath_tmpb_seq \l__tikzspath_tmpa_tl
  }

  \seq_clear:N \l__tikzspath_tmpb_seq
  \seq_map_inline:Nn \l__tikzspath_tmpa_seq {
    \seq_put_right:Nx
    \l__tikzspath_tmpb_seq
    {\int_eval:n
      {
        \int_mod:nn { ##1 }{ \l__tikzspath_tmpa_int } + 1
      }
    }
  }

  \spath_segments_to_seq:Nn \l__tikzspath_tmpc_seq {#1}

  \seq_clear:N \l__tikzspath_tmpd_seq
  \seq_map_indexed_inline:Nn \l__tikzspath_tmpc_seq
  {
    \tl_set:Nn \l__tikzspath_tmpa_tl {##2}
    \seq_if_in:NnT \l__tikzspath_tmpa_seq {##1}
    {
      \spath_shorten_at_end:Nn \l__tikzspath_tmpa_tl {(#2)/2}
    }
    \seq_if_in:NnT \l__tikzspath_tmpb_seq {##1}
    {
      \spath_shorten_at_start:Nn \l__tikzspath_tmpa_tl {(#2)/2}
    }
    \seq_put_right:NV \l__tikzspath_tmpd_seq \l__tikzspath_tmpa_tl
  }
  \tl_gset:Nx \g__tikzspath_output_tl {\seq_use:Nn \l__tikzspath_tmpd_seq {} }
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_insert_gaps_after_segments:Nnnn #1#2#3#4
{
  \__tikzspath_insert_gaps_after_segments_aux:nnn {#2}{#3}{#4}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_insert_gaps_after_segments:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_insert_gaps_after_segments:Nnn #1#2#3
{
  \__tikzspath_insert_gaps_after_segments:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_insert_gaps_after_segments:Nnn {cnn, cVV}
\cs_new_protected_nopar:Npn \__tikzspath_ginsert_gaps_after_segments:Nnnn #1#2#3#4
{
  \__tikzspath_insert_gaps_after_segments_aux:nnn {#2}{#3}{#4}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_ginsert_gaps_after_segments:Nnnn {NVnn}
\cs_new_protected_nopar:Npn \__tikzspath_ginsert_gaps_after_segments:Nnn #1#2#3
{
  \__tikzspath_ginsert_gaps_after_segments:NVnn #1#1{#2}{#3}
}
\cs_generate_variant:Nn \__tikzspath_ginsert_gaps_after_segments:Nnn {cnn, cVV}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_aux:nn #1#2
{
  \group_begin:

  \tl_set:Nn \l__tikzspath_tmpa_tl {#1}
  \spath_numberofcomponents:NV \l__tikzspath_tmpa_int \l__tikzspath_tmpa_tl
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_int {#2}

  \seq_reverse:N \l__tikzspath_tmpa_seq

  \seq_map_inline:Nn \l__tikzspath_tmpa_seq
  {
    \spath_join_component:Nn \l__tikzspath_tmpa_tl {##1}
  }
  \tl_gset_eq:NN \g__tikzspath_output_tl \l__tikzspath_tmpa_tl
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_join_components:Nnn #1#2#3
{
  \__tikzspath_join_components_aux:nn {#2}{#3}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_join_components:Nnn {NVn}
\cs_new_protected_nopar:Npn \__tikzspath_join_components:Nn #1#2
{
  \__tikzspath_join_components:NVn #1#1{#2}
}
\cs_generate_variant:Nn \__tikzspath_join_components:Nn {cn}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components:Nnn #1#2#3
{
  \__tikzspath_join_components_aux:nn {#2}{#3}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components:Nnn {NVn}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components:Nn #1#2
{
  \__tikzspath_gjoin_components:NVn #1#1{#2}
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components:Nn {cn}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_with_bezier_aux:nn #1#2
{
  \group_begin:
  \tl_set:Nn \l__tikzspath_tmpc_tl {#1}
  \tl_if_empty:nT {#2}
  {
    \spath_spot_weld_components:N \l__tikzspath_tmpc_tl
  }

  \spath_numberofcomponents:NV \l__tikzspath_tmpa_int \l__tikzspath_tmpc_tl
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpb_seq \l__tikzspath_tmpa_int {#2}

  \spath_components_to_seq:NV \l__tikzspath_tmpa_seq \l__tikzspath_tmpc_tl

  \seq_pop_left:NN \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_tl
  \seq_pop_left:NN \l__tikzspath_tmpb_seq \l__tikzspath_tmpb_tl

  \seq_map_indexed_inline:Nn \l__tikzspath_tmpa_seq
  {
    \int_compare:nTF
    {
      ##1 == \l__tikzspath_tmpb_tl
    }
    {
      \seq_pop_left:NNF \l__tikzspath_tmpb_seq \l__tikzspath_tmpb_tl
      {
        \tl_set:Nn \l__tikzspath_tmpb_tl {-1}
      }
      \spath_curve_between:Nn \l__tikzspath_tmpa_tl {##2}
    }
    {
      \tl_put_right:Nn \l__tikzspath_tmpa_tl {##2}
    }
  }
  \tl_gset_eq:NN \g__tikzspath_output_tl \l__tikzspath_tmpa_tl
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_with_bezier:Nnn #1#2#3
{
  \__tikzspath_join_components_with_bezier_aux:nn {#2}{#3}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_join_components_with_bezier:Nnn {NVn}
\cs_new_protected_nopar:Npn \__tikzspath_join_components_with_bezier:Nn #1#2
{
  \__tikzspath_join_components_with_bezier:NVn #1#1{#2}
}
\cs_generate_variant:Nn \__tikzspath_join_components_with_bezier:Nn {cV}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components_with_bezier:Nnn #1#2#3
{
  \__tikzspath_join_components_with_bezier_aux:nn {#2}{#3}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components_with_bezier:Nnn {NVn}
\cs_new_protected_nopar:Npn \__tikzspath_gjoin_components_with_bezier:Nn #1#2
{
  \__tikzspath_gjoin_components_with_bezier:NVn #1#1{#2}
}
\cs_generate_variant:Nn \__tikzspath_gjoin_components_with_bezier:Nn {cV}
\cs_new_protected_nopar:Npn \__tikzspath_remove_components_aux:nn #1#2
{
  \group_begin:

  \spath_numberofcomponents:Nn \l__tikzspath_tmpa_int {#1}
  \__tikzspath_seq_from_foreach:NVn \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_int {#2}

  \spath_components_to_seq:Nn \l__tikzspath_tmpb_seq {#1}

  \seq_pop_left:NNF \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_tl
  {
    \tl_clear:N \l__tikzspath_tmpa_tl
  }

  \seq_clear:N \l__tikzspath_tmpc_seq
  \seq_map_indexed_inline:Nn \l__tikzspath_tmpb_seq
  {
    \tl_set:Nn \l__tikzspath_tmpb_tl {##1}
    \tl_if_eq:NNTF \l__tikzspath_tmpb_tl \l__tikzspath_tmpa_tl
    {
      \seq_pop_left:NNF \l__tikzspath_tmpa_seq \l__tikzspath_tmpa_tl
      {
        \tl_clear:N \l__tikzspath_tmpa_tl
      }
    }
    {
      \seq_put_right:Nn \l__tikzspath_tmpc_seq {##2}
    }
  }

  \tl_gset:Nx \g__tikzspath_output_tl {\seq_use:Nn \l__tikzspath_tmpc_seq {} }
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_remove_components:Nnn #1#2#3
{
  \__tikzspath_remove_components_aux:nn {#2}{#3}
  \tl_set_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_remove_components:Nnn {NVn}
\cs_new_protected_nopar:Npn \__tikzspath_remove_components:Nn #1#2
{
  \__tikzspath_remove_components:NVn #1#1{#2}
}
\cs_generate_variant:Nn \__tikzspath_remove_components:Nn {cn}
\cs_new_protected_nopar:Npn \__tikzspath_gremove_components:Nnn #1#2#3
{
  \__tikzspath_remove_components_aux:nn {#2}{#3}
  \tl_gset_eq:NN #1 \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_gremove_components:Nnn {NVn}
\cs_new_protected_nopar:Npn \__tikzspath_gremove_components:Nn #1#2
{
  \__tikzspath_gremove_components:NVn #1#1{#2}
}
\cs_generate_variant:Nn \__tikzspath_gremove_components:Nn {cn}
\cs_new_protected_nopar:Npn \__tikzspath_transform_to_aux:nn #1#2
{
  \group_begin:
  \spath_reallength:Nn \l__tikzspath_tmpa_int {#2}

  \tl_set:Nx \l__tikzspath_tmpb_tl
  {\fp_to_decimal:n {(#1) * (\l__tikzspath_tmpa_int)}}
  \spath_transformation_at:NnV \l__tikzspath_tmpc_tl {#2} \l__tikzspath_tmpb_tl
  \tl_gset_eq:NN \g__tikzspath_output_tl \l__tikzspath_tmpc_tl
  \group_end:
}
\cs_new_protected_nopar:Npn \__tikzspath_transform_to:nn #1#2
{
  \__tikzspath_transform_to_aux:nn {#1}{#2}
  \exp_last_unbraced:NV \pgfsettransformentries \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_transform_to:nn {nv}
\cs_new_protected_nopar:Npn \__tikzspath_transform_upright_to:nn #1#2
{
  \__tikzspath_transform_to_aux:nn {#1}{#2}
  \fp_compare:nT { \tl_item:Nn \g__tikzspath_output_tl {4} < 0}
  {
    \tl_gset:Nx \g__tikzspath_output_tl
    {
      { \fp_eval:n { - (\tl_item:Nn \g__tikzspath_output_tl {1})} }
      { \fp_eval:n { - (\tl_item:Nn \g__tikzspath_output_tl {2})} }
      { \fp_eval:n { - (\tl_item:Nn \g__tikzspath_output_tl {3})} }
      { \fp_eval:n { - (\tl_item:Nn \g__tikzspath_output_tl {4})} }
      { \tl_item:Nn \g__tikzspath_output_tl {5} }
      { \tl_item:Nn \g__tikzspath_output_tl {6} }
    }
  }
  \exp_last_unbraced:NV \pgfsettransformentries \g__tikzspath_output_tl
  \tl_gclear:N \g__tikzspath_output_tl
}
\cs_generate_variant:Nn \__tikzspath_transform_upright_to:nn {nv}
\tikzset{
  spath/.is~family,
  spath/.cd,
  set~ prefix/.store~ in=\l__tikzspath_prefix_tl,
  prefix/.is~choice,
  prefix/default/.style={
    /tikz/spath/set~ prefix=tikz@intersect@path@name@
  },
  set~ suffix/.store~ in=\l__tikzspath_suffix_tl,
  suffix/.is~choice,
  suffix/default/.style={
    /tikz/spath/set~ suffix={}
  },
  set~ name/.style={
    /tikz/spath/prefix=#1,
    /tikz/spath/suffix=#1
  },
  at~ end~ path~ construction/.code={
    \tl_put_right:Nn \l__tikzspath_tikzpath_finish_tl {#1}
  },
  save/.code={
    \tikz@addmode{
      \spath_get_current_path:N \l__tikzspath_tmpa_tl
      \spath_bake_round:NV \l__tikzspath_tmpa_tl \l__tikzspath_tmpa_tl
      \spath_bake_shorten:NV \l__tikzspath_tmpa_tl \l__tikzspath_tmpa_tl
      \spath_save_path:cV {\__tikzspath_path_name:n {#1}}
      \l__tikzspath_tmpa_tl
    }
  },
  save~ global/.code={
    \tikz@addmode{
      \spath_get_current_path:N \l__tikzspath_tmpa_tl
      \spath_bake_round:NV \l__tikzspath_tmpa_tl \l__tikzspath_tmpa_tl
      \spath_bake_shorten:NV \l__tikzspath_tmpa_tl \l__tikzspath_tmpa_tl
      \spath_gsave_path:cV {\__tikzspath_path_name:n {#1}}
      \l__tikzspath_tmpa_tl
    }
  },
  clone/.code~ 2~ args={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \tl_clear_new:c {\__tikzspath_path_name:n {#1}}
        \tl_set_eq:cc {\__tikzspath_path_name:n {#1}}
      }
    }
    {#2}{}
  },
  clone~ global/.code~ 2~ args={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \tl_gclear_new:c {\__tikzspath_path_name:n {#1}}
        \tl_gset_eq:cc {\__tikzspath_path_name:n {#1}}
      }
    }
    {#2}{}
  },
  save~ to~ aux/.code={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \spath_save_to_aux:c
      }
    }
    {#1}
    {}
  },
  export~ to~ svg/.code={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \spath_export_to_svg:nv {#1}
      }
    }
    {#1}
    {}
  },
  use/.code={
    \bool_set_false:N \l__tikzspath_reverse_bool
    \bool_set_false:N \l__tikzspath_weld_bool
    \bool_set_false:N \l__tikzspath_move_bool
    \bool_set_false:N \l__tikzspath_current_transformation_bool
    \bool_set_true:N \l_spath_movetorelevant_bool
    \tl_clear:N \l__tikzspath_joinpath_tl
    \tl_clear:N \l__tikzspath_transformation_tl
    \tikzset{
      spath/join/.cd,
      #1
    }

    \__tikzspath_check_path:nVn
    {
      \__tikzspath_use_path:v
    } \l__tikzspath_joinpath_tl {}

  },
  restore/.style={/tikz/spath/use={#1}},
  restore~ reverse/.style={/tikz/spath/use={reverse, #1}},
  append/.style={/tikz/spath/use={move, weld, #1}},
  append~ no~ move/.style={/tikz/spath/use={weld, #1}},
  append~ reverse/.style={/tikz/spath/use={move, weld, reverse, #1}},
  append~ reverse~ no~ move/.style={/tikz/spath/use={weld, reverse, #1}},
  insert/.style={/tikz/spath/use={#1}},
  insert~ reverse/.style={/tikz/spath/use={reverse, #1}},
  show~current~path/.code={
    \tikz@addmode{
      \pgfsyssoftpath@getcurrentpath\l__tikzspath_tmpa_tl
      \iow_term:n {---~ current~ soft~ path~ ---}
      \spath_show:V \l__tikzspath_tmpa_tl
    }
  },
  show/.code={
    \__tikzspath_check_path:nnn {
      \iow_term:n {---~ soft~ path~ #1~ ---}
      \spath_show:v
    } {#1} {}
  },
  join~ with/.code~ 2~ args={
    \bool_set_false:N \l__tikzspath_reverse_bool
    \bool_set_false:N \l__tikzspath_weld_bool
    \bool_set_false:N \l__tikzspath_move_bool
    \bool_set_false:N \l__tikzspath_global_bool
    \bool_set_false:N \l__tikzspath_current_transformation_bool
    \tl_clear:N \l__tikzspath_joinpath_tl
    \tl_clear:N \l__tikzspath_transformation_tl
    \tikzset{
      spath/join/.cd,
      #2
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnVn
      {
        \__tikzspath_join_with:cv
      }
    } {#1} { \l__tikzspath_joinpath_tl {} }
  },
  spot~ weld/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_spot_weld_components:c
      }
    } {#1} { {} }
  },
  spot~ weld~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_spot_gweld_components:c
      }
    } {#1} { {} }
  },
  reverse/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_reverse:c
      }
    } {#1} { {} }
  },
  reverse~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_greverse:c
      }
    } {#1} { {} }
  },
  span/.code ~n~ args={3}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_process_tikz_point:Nn \l__tikzspath_tmpa_tl {#2}
        \__tikzspath_process_tikz_point:Nn \l__tikzspath_tmpb_tl {#3}
        \spath_span:cVV
      }
    } {#1} { {} \l__tikzspath_tmpa_tl \l__tikzspath_tmpb_tl }
  },
  span~ global/.code ~n~ args={3}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_process_tikz_point:Nn \l__tikzspath_tmpa_tl {#2}
        \__tikzspath_process_tikz_point:Nn \l__tikzspath_tmpb_tl {#3}
        \spath_span:cVV
      }
    } {#1} { {} \l__tikzspath_tmpa_tl \l__tikzspath_tmpb_tl }
  },
  to/.style={
    to~path={
      [
        spath/span={#1}{(\tikztostart)}{(\tikztotarget)},
        spath/use={#1,weld},
      ]
      \tikztonodes
    }
  },
  splice/.code ~n~ args={3}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_three_paths:nnnnn
      {
        \spath_splice_between:cvv
      }
    } {#1} { {#2} {#3} {} }
  },
  splice~ global/.code ~n~ args={3}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_three_paths:nnnnn
      {
        \spath_gsplice_between:cvv
      }
    } {#1} { {#2} {#3} {} }
  },
  join~ components~ with/.code~2~args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnVn
      {
        \__tikzspath_join_components_with:cvV
      }
    } {#1} { \l__tikzspath_tmpc_tl {} \l__tikzspath_tmpd_tl  }
  },
  join~ components~ globally~ with/.code~2~args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnVn
      {
        \__tikzspath_gjoin_components_with:cvV
      }
    } {#1} { \l__tikzspath_tmpc_tl {} \l__tikzspath_tmpd_tl  }
  },
  join~ components~ upright~ with/.code~2~args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnVn
      {
        \__tikzspath_join_components_upright_with:cvV
      }
    } {#1} { \l__tikzspath_tmpc_tl {} \l__tikzspath_tmpd_tl  }
  },
  join~ components~ globally~ upright~ with/.code~2~args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnVn
      {
        \__tikzspath_gjoin_components_upright_with:cvV
      }
    } {#1} { \l__tikzspath_tmpc_tl {} \l__tikzspath_tmpd_tl  }
  },
  join~ components~ with~ bezier/.code={
    \tl_if_head_is_group:nTF {#1}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#1} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#1} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#1}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nVn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_join_components_with_bezier:cV
      }
    } \l__tikzspath_tmpc_tl { {} \l__tikzspath_tmpd_tl }
  },
  join~ components~ globally~ with~ bezier/.code~2~args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_gjoin_components_with_bezier:cn
      }
    } {#1} { {} {#2} }
  },
  close/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_close:c
      }
    } {#1} { {} }
  },
  close~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gclose:c
      }
    } {#1} { {} }
  },
  open/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_open:c
      }
    } {#1} { {} }
  },
  open~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gopen:c
      }
    } {#1} { {} }
  },
  adjust~ and~ close/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_adjust_close:c
      }
    } {#1} { {} }
  },
  adjust~ and~ close~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_adjust_gclose:c
      }
    } {#1} { {} }
  },
  close~ with/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnnn
      {
        \spath_close_with:cv
      }
    } {#1} { {#2} {} }
  },
  close~ globally~ with/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_two_paths:nnnn
      {
        \spath_gclose_with:cv
      }
    } {#1} { {#2} {} }
  },
  close~ with~ curve/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_close_with_curve:c
      }
    } {#1} { {} }
  },
  close~ globally~ with~ curve/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gclose_with_curve:c
      }
    } {#1} { {} }
  },
  shorten~ at~ end/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_shorten_at_end:cn
      }
    } {#1} { {} {#2} }
  },
  shorten~ at~ start/.code~ 2~ args ={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_shorten_at_start:cn
      }
    } {#1} { {} {#2} }
  },
  shorten~ at~ both~ ends/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_shorten_at_both_ends:cn
      }
    } {#1} { {} {#2} }
  },
  shorten~ globally~ at~ end/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gshorten_at_end:cn
      }
    } {#1} { {} {#2} }
  },
  shorten~ globally~ at~ start/.code~ 2~ args ={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gshorten_at_start:cn
      }
    } {#1} { {} {#2} }
  },
  shorten~ globally~ at~ both~ ends/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gshorten_at_both_ends:cn
      }
    } {#1} { {} {#2} }
  },
  split~ at/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_split_at_normalised:cn
      }
    } {#1} { {} {#2} }
  },
  split~ globally~ at/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gsplit_at_normalised:cn
      }
    } {#1} { {} {#2} }
  },
  split~ at~ into/.code~ n~ args={4}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_split_at_normalised:ccvn {\__tikzspath_path_name:n {#1}}
        {\__tikzspath_path_name:n {#2}}
      }
    } {#3} { {} {#4} }
  },
  split~ globally~ at~ into/.code~ n~ args={4}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gsplit_at_normalised:ccvn {\__tikzspath_path_name:n {#1}}
        {\__tikzspath_path_name:n {#2}}
      }
    } {#3} { {} {#4} }
  },
  split~ at~ keep~ start/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_split_at_normalised_keep_start:cn
      }
    } {#1} { {} {#2} }
  },
  split~ globally~ at~ keep~ start/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gsplit_at_normalised_keep_start:cn
      }
    } {#1} { {} {#2} }
  },
  split~ at~ keep~ end/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_split_at_normalised_keep_end:cn
      }
    } {#1} { {} {#2} }
  },
  split~ globally~ at~ keep~ end/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gsplit_at_normalised_keep_end:cn
      }
    } {#1} { {} {#2} }
  },
  split~ at~ keep~ middle/.style~ n~ args={3}{
    /tikz/spath/split~ at~ keep~ start={#1}{#3},
    /tikz/spath/split~ at~ keep~ end={#1}{(#2)/(#3)},
  },
  split~ globally~ at~ keep~ middle/.style~ n~ args={3}{
    /tikz/spath/split~ globally~ at~ keep~ start={#1}{#3},
    /tikz/spath/split~ globally~ at~ keep~ end={#1}{(#2)/(#3)},
  },
  translate/.code~ n~ args={3}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_translate:cnn
      }
    } {#1} { {} {#2}{#3} }
  },
  translate~ globally/.code~ n~ args={3}{
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gtranslate:cnn
      }
    } {#1} { {} {#2}{#3} }
  },
  normalise/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_normalise:c
      }
    } {#1} { {} }
  },
  normalise~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gnormalise:c
      }
    } {#1} { {} }
  },
  transform/.code~ 2~ args={
    \group_begin:
    \pgftransformreset
    \tikzset{#2}
    \pgfgettransform \l__tikzspath_tmpa_tl
    \tl_gset_eq:NN \g__tikzspath_smuggle_tl \l__tikzspath_tmpa_tl
    \group_end:

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_transform:cV
      }
    } {#1} { {} \g__tikzspath_smuggle_tl }
  },
  transform~globally/.code~ 2~ args={
    \group_begin:
    \pgftransformreset
    \tikzset{#2}
    \pgfgettransform \l__tikzspath_tmpa_tl
    \tl_gset_eq:NN \g__tikzspath_smuggle_tl \l__tikzspath_tmpa_tl
    \group_end:

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gtransform:cV
      }
    } {#1} { {} \g__tikzspath_smuggle_tl }
  },
  split~ at~ intersections~ with/.code~ 2~ args={
    \tl_if_exist:cTF
    {
      tikz@library@intersections@loaded
    }
    {
      \__tikzspath_maybe_current_two_paths_reuse_first:nnnn
      {
        \__tikzspath_check_two_paths:nnnn
        {
          \spath_split_path_at_intersections:cv
        }
      } {#1} {#2} { {} }
    }
    {
      \msg_warning:nn { spath3 } { load intersections }
    }
  },
  split~ globally~ at~ intersections~ with/.code~ n~ args={2}{
    \tl_if_exist:cTF
    {
      tikz@library@intersections@loaded
    }
    {
      \__tikzspath_maybe_current_two_paths_reuse_first:nnnn
      {
        \__tikzspath_check_two_paths:nnnn
        {
          \spath_gsplit_path_at_intersections:cv
        }
      } {#1} {#2} { {} }
    }
    {
      \msg_warning:nn { spath3 } { load intersections }
    }
  },
  split~ at~ intersections/.code~ n~ args={2}{
    \tl_if_exist:cTF
    {
      tikz@library@intersections@loaded
    }
    {
      \__tikzspath_maybe_current_two_paths_reuse_both:nnnn
      {
        \__tikzspath_check_two_paths:nnnn
        {
          \spath_split_at_intersections:cc
        }
      } {#1} {#2} { {} }
    }
    {
      \msg_warning:nn { spath3 } { load intersections }
    }
  },
  split~ globally~ at~ intersections/.code~ n~ args={2}{
    \tl_if_exist:cTF
    {
      tikz@library@intersections@loaded
    }
    {
      \__tikzspath_maybe_current_two_paths_reuse_both:nnnn
      {
        \__tikzspath_check_two_paths:nnnn
        {
          \spath_gsplit_at_intersections:cc
        }
      } {#1} {#2} { {} }
    }
    {
      \msg_warning:nn { spath3 } { load intersections }
    }
  },
  split~ at~ self~ intersections/.code={
    \tl_if_exist:cTF
    {
      tikz@library@intersections@loaded
    }
    {
      \__tikzspath_maybe_current_path_reuse:nnn
      {
        \__tikzspath_check_path:nnn
        {
          \spath_split_at_self_intersections:c
        }
      } {#1} { {} }
    }
    {
      \msg_warning:nn { spath3 } { load intersections }
    }
  },
  split~ globally~ at~ self~ intersections/.code={
    \tl_if_exist:cTF
    {
      tikz@library@intersections@loaded
    }
    {
      \__tikzspath_maybe_current_path_reuse:nnn
      {
        \__tikzspath_check_path:nnn
        {
          \spath_gsplit_at_self_intersections:c
        }
      } {#1} { {} }
    }
    {
      \msg_warning:nn { spath3 } { load intersections }
    }
  },
  get~ components~ of/.code~ 2~ args={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \__tikzspath_get_components:Nv #2
      }
    }
    {#1}
    {}
  },
  get~ components~ of~ globally/.code~ 2~ args={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \__tikzspath_gget_components:Nv #2
      }
    }
    {#1}
    {}
  },
  render~ components/.code={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \__tikzspath_render_components:nv {#1}
      }
    }
    {#1}
    {}
  },
  insert~ gaps~ after~ components/.code~ 2~ args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_insert_gaps_after_components:cVV
      }
    } {#1} { {} \l__tikzspath_tmpc_tl \l__tikzspath_tmpd_tl  }
  },
  insert~ gaps~ globally~ after~ components/.code~ 2~ args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_ginsert_gaps_after_components:cVV
      }
    } {#1} { {} \l__tikzspath_tmpc_tl \l__tikzspath_tmpd_tl  }
  },
  insert~ gaps~ after~ segments/.code~ 2~ args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_insert_gaps_after_segments:cVV
      }
    } {#1} { {} \l__tikzspath_tmpc_tl \l__tikzspath_tmpd_tl  }
  },
  insert~ gaps~ globally~ after~ segments/.code~ 2~ args={
    \tl_if_head_is_group:nTF {#2}
    {
      \tl_set:Nx \l__tikzspath_tmpc_tl { \tl_item:nn {#2} {1} }
      \tl_set:Nx \l__tikzspath_tmpd_tl { \tl_item:nn {#2} {2} }
    }
    {
      \tl_set:Nn \l__tikzspath_tmpc_tl {#2}
      \tl_clear:N \l__tikzspath_tmpd_tl
    }

    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_ginsert_gaps_after_segments:cVV
      }
    } {#1} { {} \l__tikzspath_tmpc_tl \l__tikzspath_tmpd_tl  }
  },
  join~ components/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_join_components:cn
      }
    } {#1} { {} {#2} }
  },
  join~ components~ globally/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_gjoin_components:cn
      }
    } {#1} { {} {#2} }
  },
  remove~ empty~ components/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_remove_empty_components:c
      }
    } {#1} { {} }
  },
  remove~ empty~ components~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_gremove_empty_components:c
      }
    } {#1} { {} }
  },
  replace~ lines/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_replace_lines:c
      }
    } {#1} { {} }
  },
  replace~ lines~ globally/.code={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \spath_greplace_lines:c
      }
    } {#1} { {} }
  },
  remove~ components/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_remove_components:cn
      }
    } {#1} { {} {#2} }
  },
  remove~ components~ globally/.code~ 2~ args={
    \__tikzspath_maybe_current_path_reuse:nnn
    {
      \__tikzspath_check_path:nnn
      {
        \__tikzspath_gremove_components:cn
      }
    } {#1} { {} {#2} }
  },
  draft~ mode/.is~ choice,
  draft~ mode/true/.code={
    \bool_set_true:N \l__tikzspath_draft_bool
  },
  draft~ mode/false/.code={
    \bool_set_false:N \l__tikzspath_draft_bool
  },
  maybe~ spot~ weld/.code={
    \bool_if:NF \l__tikzspath_draft_bool
    {
      \__tikzspath_maybe_current_path_reuse:nnn
      {
        \__tikzspath_check_path:nnn
        {
          \spath_spot_weld_components:c
        }
      } {#1} { {} }
    }
  },
  maybe~ spot~ weld~ globally/.code={
    \bool_if:NF \l__tikzspath_draft_bool
    {
      \__tikzspath_maybe_current_path_reuse:nnn
      {
        \__tikzspath_check_path:nnn
        {
          \spath_spot_gweld_components:c
        }
      } {#1} { {} }
    }
  },
  transform~ to/.code~ 2~ args={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \__tikzspath_transform_to:nv {#2}
      }
    }
    {#1}
    {
      \pgfsettransformentries {1}{0}{0}{1}{0pt}{0pt}
    }
  },
  upright~ transform~ to/.code~ 2~ args={
    \__tikzspath_maybe_current_path:nn
    {
      \__tikzspath_check_path:nnn {
        \__tikzspath_transform_upright_to:nv {#2}
      }
    }
    {#1}
    {
      \pgfsettransformentries {1}{0}{0}{1}{0pt}{0pt}
    }
  },
  knot/.style~ n~ args={3}{
    /tikz/spath/split~ at~ self~ intersections=#1,
    /tikz/spath/remove~ empty~ components=#1,
    /tikz/spath/insert~ gaps~ after~ components={#1}{#2}{#3},
    /tikz/spath/maybe~ spot~ weld=#1,
    /tikz/spath/render~ components=#1
  },
  global~ knot/.style~ n~ args={3}{
    /tikz/spath/split~ globally~ at~ self~ intersections=#1,
    /tikz/spath/remove~ empty~ components~ globally=#1,
    /tikz/spath/insert~ gaps~ globally ~after~ components={#1}{#2}{#3},
    /tikz/spath/maybe~ spot~ weld~ globally=#1,
    /tikz/spath/render~ components=#1
  },
  show/.default=current,
  spot~ weld/.default=current,
  spot~ weld~ globally/.default=current,
  reverse/.default=current,
  reverse~ globally/.default=current,
  close/.default=current,
  close~ globally/.default=current,
  open/.default=current,
  open~ globally/.default=current,
  adjust~ and~ close/.default=current,
  adjust~ and~ close~ globally/.default=current,
  close~ with~ curve/.default=current,
  close~ globally~ with~ curve/.default=current,
  remove~ empty~ components/.default=current,
  remove~ empty~ components~ globally/.default=current,
  replace~ lines/.default=current,
  replace~ lines~ globally/.default=current,
  maybe~ spot~ weld/.default=current,
  maybe~ spot~ weld~ globally/.default=current,
}
\cs_new_protected_nopar:Npn \__tikzspath_get_point_at:nn #1#2
{
  \group_begin:
  \spath_reallength:Nn \l__tikzspath_tmpa_int {#2}
  \tl_set:Nx \l__tikzspath_tmpb_tl
  {\fp_to_decimal:n {(#1) * (\l__tikzspath_tmpa_int)}}
  \spath_point_at:NnV \l__tikzspath_tmpc_tl {#2} \l__tikzspath_tmpb_tl

  \tl_clear:N \l__tikzspath_tmpd_tl
  \tl_put_right:Nn \l__tikzspath_tmpd_tl {\pgf@x=}
  \tl_put_right:Nx \l__tikzspath_tmpd_tl {\tl_item:Nn \l__tikzspath_tmpc_tl {1}}
  \tl_put_right:Nn \l__tikzspath_tmpd_tl {\relax}
  \tl_put_right:Nn \l__tikzspath_tmpd_tl {\pgf@y=}
  \tl_put_right:Nx \l__tikzspath_tmpd_tl {\tl_item:Nn \l__tikzspath_tmpc_tl {2}}
  \tl_put_right:Nn \l__tikzspath_tmpd_tl {\relax}

  \tl_gset_eq:NN \g__tikzspath_output_tl \l__tikzspath_tmpd_tl
  \group_end:
 }
\cs_generate_variant:Nn \__tikzspath_get_point_at:nn {VV, Vn, Vv}

\tikzdeclarecoordinatesystem{spath}{%
  \group_begin:
  \tl_set:Nn \l__tikzspath_tmpa_tl {#1}
  \tl_trim_spaces:N \l__tikzspath_tmpa_tl

  \seq_set_split:NnV \l__tikzspath_tmpa_seq {~} \l__tikzspath_tmpa_tl
  \seq_pop_right:NN \l__tikzspath_tmpa_seq \l__tikzspath_tmpb_tl

  \tl_set:Nx \l__tikzspath_tmpa_tl { \seq_use:Nn \l__tikzspath_tmpa_seq {~} }

  \__tikzspath_maybe_current_path:nV
  {
    \__tikzspath_check_path:nnn {
      \__tikzspath_get_point_at:Vv \l__tikzspath_tmpb_tl
    }
  }
  \l__tikzspath_tmpa_tl
  {
    \tl_gset_eq:NN \g__tikzspath_output_tl \pgfpointorigin
  }

  \group_end:
  \use:c {pgf@process}{%
    \tl_use:N \g__tikzspath_output_tl
    \pgftransforminvert
    \use:c {pgf@pos@transform@glob}
  }
  \tl_gclear:N \g__tikzspath_output_tl
}

\ExplSyntaxOff
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  spath3_code.dtx
%%                                  calligraphy_doc.tex
%%                                  knots_doc.tex
%%                                  spath3.tex
%% and the derived files            spath3.ins,
%%                                  spath3_code.pdf,
%%                                  spath3.sty,
%%                                  tikzlibrarycalligraphy.code.tex
%%                                  tikzlibraryknots.code.tex
%%                                  tikzlibraryspath3.code.tex
%%                                  calligraphy.pdf
%%                                  knots.pdf
%%                                  spath3.pdf
%%                                  README
%% 
%%
%% End of file `tikzlibraryspath3.code.tex'.

